LHC Forward Physics

The goal of this report is to give a comprehensive overview of the rich field of forward physics, with a special attention to the topics that can be studied at the LHC. The report starts presenting a selection of the Monte Carlo simulation tools currently available, chapter 2, then enters the rich phenomenology of QCD at low, chapter 3, and high, chapter 4, momentum transfer, while the unique scattering conditions of central exclusive production are analyzed in chapter 5. The last two experimental topics, Cosmic Ray and Heavy Ion physics are presented in the chapter 6 and 7 respectively. Chapter 8 is dedicated to the BFKL dynamics, multiparton interactions, and saturation. The report ends with an overview of the forward detectors at LHC. Each chapter is correlated with a comprehensive bibliography, attempting to provide to the interested reader with a wide opportunity for further studies.

==> detectors/AFP.tex <==
%\subsection{Introduction}

The ATLAS Forward Proton (AFP) program aims to intercept and measure protons emitted in the very forward directions from the ATLAS interaction point (IP). Forward protons are characterized by their energy fractional loss $\xi=(E - E_{beam})/E_{beam}$ and by the four-momentum transfer squared $t=(p - p_{beam})^2 \simeq (p\theta)^2$, where $E$ and $p$ characterize the forward proton, and $\theta$ is its scattering angle.

A varied physics program using forward protons becomes available with AFP: single and double diffraction measurements, Pomeron structure functions, rapidity gap survival probability, and double Pomeron exchange (DPE) and double photon exchange (DPhE) processes. The latter give access to anomalous quartic coupling measurements of interest to beyond-Standard-Model Physics signals.

The AFP detectors consist of two forward arms, with two detector station per arm located at 206~m and 214~m from the ATLAS IP. The detectors are housed inside so-called Roman Pots, stainless steel pots that are able to move inside the beam pipe aperture after stable collisions are established. The pots have thin 300~$\mu$m windows facing the beam, to minimize interactions and to enable the detectors to approach the beam as close as possible to intercept protons with energy losses as low as $\xi\simeq 1.5$\%. The upper limit to the $\xi$-acceptance is about 15\% and determined by the LHC optics and the upstream beam apertures.

Although the non-exhaustive list of AFP physics processes covers a wide range of cross sections, some of the more interesting processes are rare and require running at the highest luminosity available. Characterizing the instantaneous luminosity by the average number of interactions, $\mu$, occurring at a bunch crossing, $\mu$\ is expected to be in excess of 25 for the upcoming LHC run period and may well reach 50 or more interactions per bunch crossing.

\subsection{Beam Interface}

The AFP Beam interface of choice is the Roman Pot (RP) because of its proven service record in the ALFA and TOTEM experiments, and the acceptable additional impedance that the RP presents to the circulationg LHC beams: less than 1\%\ of the total LHC transverse impedance. This was extensively simulated by the LHC Impedance team.

The TOTEM collaboration has developed a full design of a cylindrical horizontal RP station based on the existing horizontal and vertical RP stations of TOTEM and ALFA, see the relevant chapters in this report. The AFP RP station is a single-sided horizontal cylindrical RP station virtually identical to the TOTEM design presented in this report. Differences concern the support table, which is specific to the AFP locations near the ATLAS Interaction Point 1 (IP1). Also, the RP itself has a slightly different design: whereas the TOTEM RP design has a beam window of $300 \textmu$m thick formed by a `groove' of 1.7~mm deep and 18~mm wide on the inside of the RP bottom, the AFP RP is instead flat on the inside of the RP, with a similar `groove' facing the circulating beam. Fig.~\ref{fig:AFP-RP} shows the AFP RP design. In normal operation the AFP RP will have a secondary vacuum inside the pot, and only during the installation and removal of the detectors will the inside RP pressure go to 1 bar. The AFP RP design was simulated for mechanical stability in two extreme cases: inside pressure of 1 bar, and outside vacuum, and the reverse. The maximum stress of 0.14~GPa, see Fig.~ref{fig:AFP-RP-Stresses}, is 70\% of the assumed 0.20~GPa yield strength of the 316LN Stainless Steel and occurs near the outside corners of the thin window facing the beam. The maximum displacement occurs at the center of the thin window and is approximately 0.8 mm.
\begin{figure}
\centerline{
\includegraphics[width=.45\columnwidth]{AFP-RP-29JUL14.pdf}\hspace{0.5cm}
\includegraphics[width=.45\columnwidth]{AFP-RP-Stresses-22JUL14.pdf}}
\caption{Left: the design of the AFP Roman Pot with $300~\textmu$m windows. Note the exterior `groove' forming the window facing the beam. Right: the calculated stresses in the material} \label{fig:AFP-RP}
\end{figure} 


\subsection{Silicon Tracker}

Silicon 3D description from Sebastian.

\subsection{Time-of-Flight Detector}

Because single diffraction, which produces a single forward proton, are relatively common (about 10\% of the total cross section), an interaction of high interest, say DP(h)E which yields two forward protons, may easily be faked by the occurrence of two single-diffraction interactions in the same bunch crossing. The only possible rejection of this background to DP(h)E processes is to measure the arrival time difference of the forward protons in the two arms with pico-second accuracy. For a genuine DP(h)E two-proton event, the arrival time difference of the forward protons $\Delta{t}=t_{Left arm} - t_{Right arm}$ is directly related to the interaction vertex location $z_{vertex}$ ($z$ measured along the beam from zero at the ATLAS IP and positive toward the 'Right' arm) as: $z_{vertex} = c\Delta{t}/2$. Thus, a $\sigma_t=10$~ps time-of-flight resolution translates into a $\sigma_z=2.1$~mm vertex resolution. The vertex location derived from fast timing is compared to the location measured from the ATLAS inner detector tracking; if the two locations differ, the protons stem from unrelated background events. Extensive simulations have shown that a 10~ps Time-of-Flight measurement provides a background rejection factor around 20.

The proposed AFP Time-of-Flight detectors consist of Quartz bars positioned at the Cerenkov angle with respect to the proton directions. The Cerenkov light travels up the bars and is converted to a signal by a specialized Multi-Channleel

The proposed upgrade for AFP consists of a detector with better pixelisation that is still under study and can be diamond or Si detectors.

The PMT output signal is approximately Gaussian with a 700~ps full width at half maximum (rms$\simeq 300$~ps). Photon statistics (the mean number of photo-electrons is about 10) affect the signal amplitude but preserve the shape precisely. The goal of the electronics is to preserve the signal shape information and derive the best possible timing of the signal, independent of the signal amplitude. 

The approach chosen by the AFP timing group is low-noise amplification followed by constant-fraction discrimination (CFD) and high-precision time digitization (HPTDC) and readout, see Fig.~\ref{fig:Electronics-Chain} where the various components and their locations are depicted.
\begin{figure}
\centerline{\includegraphics[width=.9\columnwidth]{ToF_FTelectronicsDiagram.pdf}}
\caption{A schematic diagram of the components of the fast timing electronics chain described in the text, together with their physical locations in the LHC tunnel. } \label{fig:Electronics-Chain}
\end{figure} 


Other approaches are possible, as discussed for example by E.~Delagnes, E.~Breton, and S.~Ritt at this workshop. Although the sampling methods described by these authors are best performing, the CFD method described here is very close to optimal, as is also shown in the overview presentation by J-F.~Genat at this workshop.

Beam tests (Fermilab 2012, CERN 2013) have shown that the single-channel resolution of PMT, Preamplifiers and CFD is 20~ps, limited by the PMT signal shape, statistics, and noise. Two or more sequential measurements (two or more successive quartz bars) will reduce the proton ToF resolution accordingly; four sequential measurements will provide 10~ps resolution.
The beauty of the system is its modularity: the resolution can be tuned by the changing the number of quartz bars in succession, while the resolution requirement per-channel is somewhat relaxed. Somewhat arbitrarily, in order to preserve the per-channel timing resolution, we require the time jitter of the electronics to be 5~ps or less.

Adjacent sequences of quartz bars cover intervals in proton energy loss $\xi$. It is assumed that the $\xi$ acceptance is subdivided into 4 intervals, each individual $\xi$ interval covered by a sequence of 2-4 quartz bars. Because the central missing mass $MM$ measured from the two protons is directly related to their $\xi$, $MM^2=\xi_1\xi_2(2E_{beam})^2$, a selection for events in which a large missing mass is produced can be formed already at the trigger level.

\subsection{Preamplifiers}
The PMT is used at a low gain of about $5\times10^4$ to maximize the lifetime of the tube in the high-rate LHC environment close to the circulating beam. The typical PMT output signal at this gain is about 8 mV for 10 photoelectrons. The AFP CFD used has a dynamic range from 250 - 1200~mV (a new design is in the works with a further improvement anticipated in dynamic range). 

In order to match the CFD dynamic range, and to provide for gain variations as function of PMT pixel and ageing, the preamplification iS done in two 20~dB stages. The first stage PA-a is located directly on the base of the PMT. The 8-channel preamplifier PCB is based on the PSA4-5043+ low-noise (NF=0.7~dB) InGaP E-PHEMT MMIC gain block (gain 18.6 dB at 1 GHz) from MiniCircuits.com, see Fig.~\ref{fig:PA-a}.
\begin{figure}
\centerline{\includegraphics[width=.9\columnwidth]{ToF_PA-a.pdf}}
\caption{The schematic diagram, layout, and photo of the low noise pre-amplifier, to be located on the photodetector base in the secondary vacuum.}
\label{fig:PA-a}
\end{figure}
The PA-a has been tested under power and demonstrated to be radiation tolerant to at least 9~kGy (LANSCE, February 2014 run with 800 MeV protons, $2.2\times10^{13}$~p/cm$^2$); this dose corresponds to the dose expected at the preamplifier location for 300~fb$^{-1}$ or three years at a luminosity of $10^{34}$~cm$^{-2}$s$^{-1}$.

The first preamplifier stage is connected by coaxial cable to the second preamplification stage (PA-b) located at floor level below the detector, where the high-energy proton flux is expected to be a factor 20 lower (the low energy neutron flux is a factor 10 lower there). 

The PA-b provides DC power (5 V) to the PA-a via the coaxial connection. The PA-b further  includes (in order): a programmable 3-bit attenuator (Hittite HMC288MS8 2 dB LSB GaAs MMIC, range 1~dB - 15~dB ), a 2 Way-$0^o$ splitter (MiniCircuits TCP-2-33W+, $-4$~dB insertion loss) providing a trigger pick-off, and a ADL5611 gain block (Analog Devices, gain 22(20)~dB at 1(4) GHz), see Fig.~\ref{fig:PA-b}. The PA-b has successfully survived the same irradiation runs and doses as PA-a.
\begin{figure}
\centerline{\includegraphics[width=.9\columnwidth]{PA-b_v302_Schematic.pdf}}
\caption{The schematic diagram of the new second-stage variable-gain amplifier PA-b, to be located below the detector at floor level.}
\label{fig:PA-b}
\end{figure}


\subsection{Trigger}
A trigger board has been designed and will be produced in the near future. The design is based on the 8-channel GaAs Discriminator MMIC 'NINO' (developed and produced by CERN, see http://knowledgetransfer.web.cern.ch/technology-transfer/external-partners/nino), followed by programmable majority circuitry to form a 'N out of M' type trigger combination on two LVPECL outputs. The option to include a (properly timed) bunch crossing gate (LVPECL) is implemented. The PCB has been laid out but not yet been produced.

The trigger signals from several adjacent quartz bar sequences are combined into a bit stream and sent over fast air-core coax cables to the ATLAS Central Trigger Processor. The trigger information from the two AFP arms can be used to form a large proton-proton 'missing mass' trigger and can be combined with various central ATLAS trigger terms.

\subsection{Constant Fraction Discriminator}
The Constant Fraction Discriminator principle has long be used to correct for time walk in cases where the signal fluctuates in amplitude but is constant in shape. The AFP design was initially developed for FP420 by Luc Bonnet of the Universit\'{e} Catholique de Louvain, and was further developed for AFP by the HEP group (J.~Pinfold, S-L.~Liu) at the University of Alberta at Edmonton (Alberta). The measured time-walk is 5~ps or less over the range 250 - 1200~mV. The design is currently revisited to obtain a larger dynamic range and to implement a time-over-threshold functionality, which will allow off-line timing corrections if so required. Moreover, the new CFD design includes an optional bunch crossing gate to reduce output rates.

A single CFD channel is implemented on a small $28\times70$~mm$^2$ daughter board, with RF I/O connectors for signal in and signal NIM out, and differential LVPECL outputs.

\subsection{High Precision Time Digitizer}
The High Precision Time Digitizer board, HPTDC, was developed by Alberta. The 12-channel board uses 4 HPTDC ASICs developed and produced by CERN in 0.25~$\mu$m CMOS technology (HPTDC, J.~Christiansen et al., http://tdc.web.cern.ch/tdc/hptdc/hptdc.htm). The four ASICs are controlled by an on-board FPGA which also handles the flow of data and controls. This and previous versions of the HPTDC board have been used successfully at various beam tests. The HPTDC, and new developments are presented by Jim Pinfold at this workshop.

The intrinsic resolution of the current HPTDC is 16~ps, which is a significant contributor to the per-channel resolution. However, new HPTDC ASIC development with smaller feature size are ongoing at CERN and may lead to significant improvements in the near future. Note that the 16~ps resolution of the HPTDC is per channel and that the contribution for a system of four quartz bars in sequence would only be 8~ps. 

The radiation tolerance of the HPTDC is not guaranteed. The HPTDC ASIC is expected to be radiation tolerant to a degree sufficient for it to be located on the tunnel floor, near the the detectors. The FPGA firmware must be re-designed to provide the appropriate checking of HPTDC registers for upsets. Moreover, the FPGA itself has to be radiation tolerant, which can be done by choosing a radiation-hard part (expensive!) or going to a fuse-programmable part. Alternatively, the FPGA can be programmed to do self-checking and organized with majority decisions in critical paths. It is the latter choice that will be pursued.

\subsection{Reference Clock}
A major component of any time-of-flight system using two widely separated detector arms (424~m apart measured along the beam line), is a synchronizing Reference Clock. As for other components, the requirement is that the two local detector clocks are synchronized to well within 5~ps.

The University of Texas group (A.~Brandt, V.~Shah, et al.) has developed a prototype Reference Clock based on a design originally by SLAC. Every Daughter Clock sends its signal to a central Reference Clock which produces a DC phase error signal that is read (on the same cable) by the Daughter Clock. The Daughter Clock adjusts its phase until the phase error signal is zero. 

The design is not fully complete at this time but initial tests indicate the desired performance can be reached.

In addition to the synchronized local clock, clock fanouts at the local detectors are required. We intend to implement these with high performant LVPECL Clock FanOut buffers from Micrel.

\subsection{Data Acquisition}
The Data Acquisition system currently foreseen is based on the Reconfigurable Cluster Element (RCE) computer daughterboards in the ATCA telecom standard. This system has successfully been employed for the testing of the ATLAS Intermediate B-Layer Silicon pixel detectors. Because the same Silicon sensors are used for the AFP tracker, the RCE-based DAQ system can be used essentially without any new development. However, the HPTDC board has to be interfaced to the RCE readout. This requires new FPGA firmware (also required for radiation tolerance!) as well as additions and modifications to the RCE software.

Because the RCE hardware is located in a low radiation and accessible area near the ATLAS detector, radiation tolerance is not an issue for the DAQ. 

\subsection{Conclusion}
We presented a complete fast electronics chain that will preserve the 20~ps per channel time resolution required for the AFP Time-of-Flight detectors. We presented a fast Trigger scheme for the AFP detectors which incorporates a rough measure of the proton energy loss for use in the ATLAS Central Trigger Processor.  We discuss radiation tolerance requirements and how they are met in the proposed chain.

This work was supported by U.S.\ National Science Foundation grants PHY1068677 and PHY1119200 and U.S.\ Department of Energy grant DE-SC0007054.

\endinput

=======================================
Electronics – Goals & Constraints
• preserve timing resolution of the detector: <20 ps/channel
– multiple measurements/proton ==> <10 ps/proton
– need multiplicity also for rejection of spurious background rejection!
– trade multiplicity for resolution: 4 measurements of 20 ps ? 10 ps 
• provide fast ?-bin trigger; transverse deflection x ? ?
– data rate up to 1 MHz/channel
• radiation-hardness or tolerance
– fluence/dose estimate for 100 fb–1 (1 yr @ 1034 cm–2s–1)
– FLUKA, IP primary/secondary interactions only, NO beam-gas (2~)


Fast Timing Electronics
Two methods to deal with pulse-height variations:
• CFD + TDC c
• Sampling of the (leading edge of the) pulse and time-walk correction
– see slides by J-F Genat, and many others at this workshop!


• AFP Baseline: CFD + HPTDC
– see Jim Pinfold es talk
• AFP Electronics R&D: SAMPIC

Pulse Shape and Gain Requirements
Pulse shape from UTA Laser-Lab testing (25ƒ?m pore) :?
– Gaussian, FWHM ~700 ps (trise~300 ps)
РMinimum pulse height at 2 pe, G=1E5: Vpeak~2 mV (~30 fC in 50 Ħ)

Trigger: needs ~100 fC

CFD needs: 250 – 1500 mV
– 2 mV ==> 200 mV:     40 dB
– PMT pixel variation: ~6 dB
– PMT ageing:            ~6 dB

> Need ~50 dB gain
– 2 or 4 (inverting) stages of ~20 dB each










Irradiation of AFP Electronics
• HiRad protocol: 
– Neutrons or HE protons: 1012 – 1013 /cm2;  ?: 1 – 10 kGy.
• MedRad protocol: 
– Neutrons or HE protons: 1011 – 1012 /cm2;  ?: 10 – 1 kGy.
• PA-a chips (PSA4-5043+): HiRad
• PA-b boards & trigger: MedRad
• NINO chips (trigger): MedRad
• CFD daughter boards: MedRad
• HPTDC chips: MedRad
Irradiation – Sep 2013
Irradiated at LANL Sept 2013; S. Seidel et al. (UNM), K. Gray (UTA): 








800 MeV p, ~7 cm from direct beam; passive
– dose: 6.5-8.7~1012 p/cm2, 2.3-3.1 kGy
– for 100 fb–1: ~expected for PA-a; ~50~ expected 
for PA-b and CFD
– devices are all operational after irradiation!
Irradiation @ LANSCE – Jan 2014
4-Channel Electronics Setup
• Jan 31- Feb 2 irradiation at LANSCE
• Protocol:
– Active irradiation
– up to 1.0~1013 p/cm2, in 10 steps of 1×1012 p/cm2
– i.e. 10 pulses of 1011 protons per step

January 31- Feb 2 Irradiation
People: Tim Hoffman (UTA); Sally Seidel, Martin Hoeferkamp (UNM)
Protocol: Active irradiation – keep voltages on!
– up to 1.0~1013 p/cm2, in 10 estepsf of 1~1012 p/cm2; verify operation before & after each step. 
– i.e. 1 estepf equals ~10 pulses of 1011 protons/pulse, 1 Hz, ~1 cm Ø

Early results:
– HPTDC readout did not work (cable too short) ==> 2 Channels were monitored on scope; all 4 channels were powered throughout the run.
– Irradiation up to 5.0~1013 p/cm2
– 2 monitored channels were still operating at the end of the run
Next:
– Wait for cool-off and return of parts (<2 months)
– Pre-Amps, CFDs: Re-test performance and compare with non-irradiated parts
– HPTDC chips: mount on HPTDC board and check operation
Fast ToF Electronics: we have c
Proven designs & prototype 8-ch modules for:
– Preamp on PMT (PA-a) (4~8 channels)
– 2nd stage variable-gain amp on tunnel floor (PA-b)  (2~8 channels)
– Constant Fraction Discriminator (CFD) (3~8 channels)
– High-Precision Time to Digital Converter (HPTDC)  (3 12-ch modules)











Have design for:
– Trigger pick-off and Multiplicity Trigger board (based on NINO chip)

Preamp/amp reflections
20 ns/div; need to reduce gringingh, tail, and reflection @ 20 ns
Reflection:
– Understood:
caused by 
mismatch of 
PA-b traces c
> Re-do PA-b PCB

1 ns ringing: 
– unclear, not seen 
with test pulses c 
– PMT?

To Do: Trigger – Stony Brook
on PA-b motherboard; uses signal pick-offs from PA-b
> to be simulated with final layout and prototyped
> Output driver: to be designed c

To Do: Modify CFD – U Alberta
add gLatch Enableh 

add Time-over-Thres-
hold functionality
Design Almost complete
Status Fast ToF Electronics: To Do c
• Fast, ultra-stable, long-distance reference clock (U Texas at Arlington)
– prototype working: ~5 ps jitter
– Clock fanout: to be designed & built: (U New Mexico)
• Trigger (Stony Brook):
– build prototype (Design almost complete)
– Radiation testing
– AFP trigger interface with CTF
• Modification of CFD (Alberta):
– add Time-over-Threshold functionality (Design almost complete)
– build prototype
• Modification of HPTDC (Alberta):
– Rad-tolerant design
– add ToT functionality (Design almost complete)
– build prototype
– Radiation testing
• Readout:
– Opto board (2 pc ordered)
– RCE Interface (SLAC/SBU) used for IBL tests
• DCS (?)



\end{document}



==> detectors/afp_yr.tex <==
\section{AFP}

The ATLAS Forward Proton (AFP) program aims to intercept and measure protons emitted in the very forward directions from the ATLAS interaction point (IP). 
Forward protons are characterized by their energy fractional loss $\xi=(E - E_{beam})/E_{beam}$ and by the four-momentum transfer 
squared $t=(p - p_{beam})^2 \simeq (p\theta)^2$, where $E$ and $p$ characterize the forward proton, and $\theta$ is its scattering angle.

A varied physics program using forward protons becomes available with AFP: single and double diffraction measurements, Pomeron structure 
functions, rapidity gap survival probability, and double Pomeron exchange (DPE) and double photon exchange (DPhE) processes. The latter give access to 
anomalous quartic coupling measurements of interest to beyond-Standard-Model Physics signals.

The AFP detectors consist of two forward arms, with two detector station per arm located at 206~m and 214~m from the ATLAS IP. The detectors are housed 
inside so-called Roman Pots, stainless steel pots that are able to move inside the beam pipe aperture after stable collisions are established. 
The pots have thin 300~$\mu$m windows facing the beam, to minimize interactions and to enable the detectors to approach the beam as close as 
possible to intercept protons with energy losses as low as $\xi\simeq 1.5$\%. The upper limit to the $\xi$-acceptance is about 15\% and determined by 
the LHC optics and the upstream beam apertures.

Although the non-exhaustive list of AFP physics processes covers a wide range of cross sections, some of the more interesting processes are rare and 
require running at the highest luminosity available. Characterizing the instantaneous luminosity by the average number of interactions, $\mu$, occurring at 
a bunch crossing, $\mu$\ is expected to be in excess of 25 for the upcoming LHC run period and may well reach 50 or more interactions per bunch crossing.

\subsection{Beam Interface}

The AFP Beam interface of choice is the Roman Pot (RP) because of its proven service record in the ALFA and TOTEM experiments, and the acceptable additional 
impedance that the RP presents to the circulationg LHC beams: less than 1\%\ of the total LHC transverse impedance. This was extensively simulated by the LHC Impedance team.

The TOTEM collaboration has developed a full design of a cylindrical horizontal RP station based on the existing horizontal and vertical RP stations of 
TOTEM and ALFA, see the relevant chapters in this report. The AFP RP station is a single-sided horizontal cylindrical RP station virtually identical to the 
TOTEM design presented in this report. Differences concern the support table, which is specific to the AFP locations near the ATLAS Interaction Point 1 (IP1).
 Also, the RP itself has a slightly different design: whereas the TOTEM RP design has a beam window of $300 \textmu$m thick formed by a `groove' 
 of 1.7~mm deep and 18~mm wide on the inside of the RP bottom, the AFP RP is instead flat on the inside of the RP, with a similar `groove' facing the 
 circulating beam. Fig.~\ref{fig:AFP-RP} shows the AFP RP design. In normal operation the AFP RP will have a secondary vacuum inside the pot, and only 
 during the installation and removal of the detectors will the inside RP pressure go to 1 bar. The AFP RP design was simulated for mechanical stability 
 in two extreme cases: inside pressure of 1 bar, and outside vacuum, and the reverse. The maximum stress of 0.14~GPa, see Fig.~ref{fig:AFP-RP-Stresses}, 
 is 70\% of the assumed 0.20~GPa yield strength of the 316LN Stainless Steel and occurs near the outside corners of the thin window facing the beam. 
 The maximum displacement occurs at the center of the thin window and is approximately 0.8 mm.
\begin{figure}
\centerline{
\includegraphics[width=.45\columnwidth]{figs/detector/AFP-RP-29JUL14.pdf}\hspace{0.5cm}
\includegraphics[width=.45\columnwidth]{figs/detector/AFP-RP-Stresses-22JUL14.pdf}}
\caption{Left: the design of the AFP Roman Pot with $300~\textmu$m windows. Note the exterior `groove' forming the window facing the beam. Right: the calculated stresses in the material} 
\label{fig:AFP-RP}
\end{figure} 


\subsection{Silicon Tracker}

Silicon 3D description from Sebastian.

\subsection{Time-of-Flight Detector}

Because single diffraction, which produces a single forward proton, are relatively common (about 10\% of the total cross section), 
an interaction of high interest, say DP(h)E which yields two forward protons, may easily be faked by the occurrence of two single-diffraction interactions in the same bunch crossing. The only possible rejection of this background to DP(h)E processes is to measure the arrival time difference of the forward protons in the two arms with pico-second accuracy. For a genuine DP(h)E two-proton event, the arrival time difference of the forward protons $\Delta{t}=t_{Left arm} - t_{Right arm}$ is directly related to the interaction vertex location $z_{vertex}$ ($z$ measured along the beam from zero at the ATLAS IP and positive toward the 'Right' arm) as: $z_{vertex} = c\Delta{t}/2$. Thus, a $\sigma_t=10$~ps time-of-flight resolution translates into a $\sigma_z=2.1$~mm vertex resolution. The vertex location derived from fast timing is compared to the location measured from the ATLAS inner detector tracking; if the two locations differ, the protons stem from unrelated background events. Extensive simulations have shown that a 10~ps Time-of-Flight measurement provides a background rejection factor around 20.

The proposed AFP Time-of-Flight detectors consist of Quartz bars positioned at the Cerenkov angle with respect to 
the proton directions. The Cerenkov light travels up the bars and is converted to a signal by a specialized Multi-Channleel

The PMT output signal is approximately Gaussian with a 700~ps full width at half maximum (rms$\simeq 300$~ps). 
Photon statistics (the mean number of photo-electrons is about 10) affect the signal amplitude but preserve the shape precisely. The goal of the electronics is to preserve the signal shape information and derive the best possible timing of the signal, independent of the signal amplitude. 

The approach chosen by the AFP timing group is low-noise amplification followed by constant-fraction discrimination (CFD) 
and high-precision time digitization (HPTDC) and readout, see Fig.~\ref{fig:Electronics-Chain} where the various components 
and their locations are depicted.
\begin{figure}
\centerline{\includegraphics[width=.9\columnwidth]{figs/detector/ToF_FTelectronicsDiagram.pdf}}
\caption{A schematic diagram of the components of the fast timing electronics chain described in the text, together with their physical locations in the LHC tunnel. } \label{fig:Electronics-Chain}
\end{figure} 


Other approaches are possible, as discussed for example by E.~Delagnes, E.~Breton, and S.~Ritt at this workshop. 
Although the sampling methods described by these authors are best performing, the CFD method described here is very close to optimal, 
as is also shown in the overview presentation by J-F.~Genat at this workshop.

Beam tests (Fermilab 2012, CERN 2013) have shown that the single-channel resolution of PMT, Preamplifiers and CFD is 20~ps, 
limited by the PMT signal shape, statistics, and noise. Two or more sequential measurements (two or more successive quartz bars) 
will reduce the proton ToF resolution accordingly; four sequential measurements will provide 10~ps resolution.
The beauty of the system is its modularity: the resolution can be tuned by the changing the number of quartz bars in succession, 
while the resolution requirement per-channel is somewhat relaxed. Somewhat arbitrarily, in order to preserve the per-channel timing 
resolution, we require the time jitter of the electronics to be 5~ps or less.

Adjacent sequences of quartz bars cover intervals in proton energy loss $\xi$. It is assumed that the $\xi$ acceptance is subdivided
 into 4 intervals, each individual $\xi$ interval covered by a sequence of 2-4 quartz bars. Because the central missing mass $MM$ measured from the two protons is directly related to 
 their $\xi$, $MM^2=\xi_1\xi_2(2E_{beam})^2$, a selection for events in which a large missing mass is produced can be formed already at the trigger level.

\subsection{Preamplifiers}
The PMT is used at a low gain of about $5\times10^4$ to maximize the lifetime of the tube in the high-rate LHC environment close to the circulating beam. The typical PMT output signal 
at this gain is about 8 mV for 10 photoelectrons. The AFP CFD used has a dynamic range from 250 - 1200~mV (a new design is in the works with a further improvement anticipated in dynamic range). 

In order to match the CFD dynamic range, and to provide for gain variations as function of PMT pixel and ageing, the preamplification iS done in two 20~dB stages. The first stage 
PA-a is located directly on the base of the PMT. The 8-channel preamplifier PCB is based on the PSA4-5043+ low-noise (NF=0.7~dB) InGaP E-PHEMT MMIC gain block (gain 18.6 dB at 1 GHz) 
from MiniCircuits.com, see Fig.~\ref{fig:PA-a}.
\begin{figure}
\centerline{\includegraphics[width=.9\columnwidth]{figs/detector/ToF_PA-a.pdf}}
\caption{The schematic diagram, layout, and photo of the low noise pre-amplifier, to be located on the photodetector base in the secondary vacuum.}
\label{fig:PA-a}
\end{figure}
The PA-a has been tested under power and demonstrated to be radiation tolerant to at least 9~kGy (LANSCE, February 2014 run with 800 MeV protons, $2.2\times10^{13}$~p/cm$^2$); 
this dose corresponds to the dose expected at the preamplifier location for 300~fb$^{-1}$ or three years at a luminosity of $10^{34}$~cm$^{-2}$s$^{-1}$.

The first preamplifier stage is connected by coaxial cable to the second preamplification stage (PA-b) located at floor level below the detector, where the high-energy proton 
flux is expected to be a factor 20 lower (the low energy neutron flux is a factor 10 lower there). 

The PA-b provides DC power (5 V) to the PA-a via the coaxial connection. The PA-b further  includes (in order): a programmable 3-bit attenuator 
(Hittite HMC288MS8 2 dB LSB GaAs MMIC, range 1~dB - 15~dB ), a 2 Way-$0^o$ splitter (MiniCircuits TCP-2-33W+, $-4$~dB insertion loss) providing a trigger pick-off, and a 
ADL5611 gain block (Analog Devices, gain 22(20)~dB at 1(4) GHz), see Fig.~\ref{fig:PA-b}. The PA-b has successfully survived the same irradiation runs and doses as PA-a.
\begin{figure}
\centerline{\includegraphics[width=.9\columnwidth]{figs/detector/PA-b_v302_Schematic.pdf}}
\caption{The schematic diagram of the new second-stage variable-gain amplifier PA-b, to be located below the detector at floor level.}
\label{fig:PA-b}
\end{figure}


\subsection{Trigger}
A trigger board has been designed and will be produced in the near future. The design is based on the 8-channel GaAs Discriminator MMIC 'NINO' 
(developed and produced by CERN, see http://knowledgetransfer.web.cern.ch/technology-transfer/external-partners/nino, to be moved to Ref...), followed by programmable majority circuitry 
to form a 'N out of M' type trigger combination on two LVPECL outputs. The option to include a (properly timed) bunch crossing gate (LVPECL) is implemented. The PCB has been laid out but not yet been produced. Let us notice that the upgrade SAMPIC solution will provide a trigger directly.


The trigger signals from several adjacent quartz bar sequences are combined into a bit stream and sent over fast air-core coax cables to the 
ATLAS Central Trigger Processor. The trigger information from the two AFP arms can be used to form a large proton-proton 'missing mass' trigger and can be combined 
with various central ATLAS trigger terms.

\subsection{Constant Fraction Discriminator}
The Constant Fraction Discriminator principle has long be used to correct for time walk in cases where the signal fluctuates in amplitude but is constant in shape. 
The AFP design was initially developed for FP420 by Luc Bonnet of the Universit\'{e} Catholique de Louvain, and was further developed for AFP by the HEP group (J.~Pinfold, S-L.~Liu) at 
the University of Alberta at Edmonton (Alberta). The measured time-walk is 5~ps or less over the range 250 - 1200~mV. The design is currently revisited to obtain a larger dynamic 
range and to implement a time-over-threshold functionality, which will allow off-line timing corrections if so required. Moreover, the new CFD design includes an optional bunch 
crossing gate to reduce output rates.

A single CFD channel is implemented on a small $28\times70$~mm$^2$ daughter board, with RF I/O connectors for signal in and signal NIM out, and differential LVPECL outputs.

\subsection{High Precision Time Digitizer}
The High Precision Time Digitizer board, HPTDC, was developed by Alberta. The 12-channel board uses 4 HPTDC ASICs developed and produced by CERN in 0.25~$\mu$m 
CMOS technology (HPTDC, J.~Christiansen et al., http://tdc.web.cern.ch/tdc/hptdc/hptdc.htm). The four ASICs are controlled by an on-board FPGA which also handles the 
flow of data and controls. This and previous versions of the HPTDC board have been used successfully at various beam tests. The HPTDC, and new developments are presented
 by Jim Pinfold at this workshop.

The intrinsic resolution of the current HPTDC is 16~ps, which is a significant contributor to the per-channel resolution. However, new HPTDC ASIC development
 with smaller feature size are ongoing at CERN and may lead to significant improvements in the near future. Note that the 16~ps resolution of the HPTDC is per 
 channel and that the contribution for a system of four quartz bars in sequence would only be 8~ps. 

The radiation tolerance of the HPTDC is not guaranteed. The HPTDC ASIC is expected to be radiation tolerant to a degree sufficient for it to be located on the
 tunnel floor, near the the detectors. The FPGA firmware must be re-designed to provide the appropriate checking of HPTDC registers for upsets. Moreover, the 
 FPGA itself has to be radiation tolerant, which can be done by choosing a radiation-hard part (expensive!) or going to a fuse-programmable part. Alternatively, 
 the FPGA can be programmed to do self-checking and organized with majority decisions in critical paths. It is the latter choice that will be pursued.

\subsection{Reference Clock}
A major component of any time-of-flight system using two widely separated detector arms (424~m apart measured along the beam line), is a synchronizing Reference Clock. 
As for other components, the requirement is that the two local detector clocks are synchronized to well within 5~ps.

The University of Texas group (A.~Brandt, V.~Shah, et al.) has developed a prototype Reference Clock based on a design originally by SLAC. Every Daughter Clock sends 
its signal to a central Reference Clock which produces a DC phase error signal that is read (on the same cable) by the Daughter Clock. The Daughter Clock adjusts its 
phase until the phase error signal is zero. 

The design is not fully complete at this time but initial tests indicate the desired performance can be reached.

In addition to the synchronized local clock, clock fanouts at the local detectors are required. We intend to implement these with high performant LVPECL Clock FanOut buffers from Micrel.

\subsection{Data Acquisition}
The Data Acquisition system currently foreseen is based on the Reconfigurable Cluster Element (RCE) computer daughterboards in the ATCA telecom standard. This system 
has successfully been employed for the testing of the ATLAS Intermediate B-Layer Silicon pixel detectors. Because the same Silicon sensors are used for the AFP tracker, 
the RCE-based DAQ system can be used essentially without any new development. However, the HPTDC board has to be interfaced to the RCE readout. This requires new FPGA 
firmware (also required for radiation tolerance!) as well as additions and modifications to the RCE software.

Because the RCE hardware is located in a low radiation and accessible area near the ATLAS detector, radiation tolerance is not an issue for the DAQ. 

\subsection{Conclusion}
We presented a complete fast electronics chain that will preserve the 20~ps per channel time resolution required for the AFP Time-of-Flight detectors. We presented a 
fast Trigger scheme for the AFP detectors which incorporates a rough measure of the proton energy loss for use in the ATLAS Central Trigger Processor.  
We discuss radiation tolerance requirements and how they are met in the proposed chain.

This work was supported by U.S.\ National Science Foundation grants PHY1068677 and PHY1119200 and U.S.\ Department of Energy grant DE-SC0007054.

\endinput



==> detectors/detectors_VA.tex <==
%\chapter{Forward Detector Systems at LHC}
\label{sec:forward_detector_systems}
%Version 16.11.2014

The following paragraphs describe the detector systems of the different LHC experiments optimized for the forward physics program as outlined in previous chapters of this report.
Already existing detectors are described shortly, or a reference to the detailed articles~\cite{jinst-global} is given. The newly developed components that have been integrated during the long 
shutdown 1 (LS 1) and the ongoing R\&D activities are described in more detail with possible reference to the corresponding technical design reports (TDRs) or upgrade proposals. 
The forward detector systems can in general be separated in two different types, the movable beam inserts with detectors and the standard detectors that are integrated in the central detector or 
installed in the LHC tunnel.
%


\paragraph*{Movable beam inserts with detector sensors}

The detector carriers which are integrated in the LHC beam tube and enter into the LHC beam vacuum are generically called ``movable beam inserts''. 
These beam inserts carry the detector sensors for tracking or timing and allow the approach of the  sensor to a distance down to a millimetre from the beam center. 
The movable beam inserts have to comply with LHC requirements in view of impedance, ultra high vacuum and safety. The material budget plays an important role, 
as a fraction of the secondary particles which are generated by  interaction of high energy particles  with the material of the movable beam inserts are scattered 
in the material of the supra conducting LHC magnets close by.
The beam insert design is universal and can be used in the different corresponding locations of the LHC machine.
  
The  specific LHC optics generates a specific particle occupancy pattern in the sensors integrated in the movable beam inserts, depending on both, the distance of 
the sensor relative to the corresponding interaction point and the location in the tunnel (experiment). For each experiment and location, the size and  pixelization of 
the sensor is specific and optimized accordingly and differs strongly for the high and low $\beta^{*}$ optics. The insertion of the beam inserts is a complex procedure 
requiring the close collaboration with the LHC collimator experts and the operators in the LHCC control room. In this sense the movable beam inserts become an integral element of the LHC machine.
  
The movable beam inserts are also present in the parking position during the standard runs and interfere with the LHC machine mostly due to their impedance. 
The beam-induced heating of the movable beam device can lead to local vacuum degradation and thus create perturbations of the machine operation during the energy ramp-up phase and the 
later stable operation of the LHC machine.    

 
\paragraph*{Standard detectors}

The standard detector for LHC forward physics can be either integrated in the central detector of an LHC experiment, or in the tunnel of LHC, outside of the vacuum beam pipe. 
The operation of these detectors is in the autonomy of the experiment. 

 
\paragraph*{Considerations for the Design and Operation of Forward Detectors at LHC with High and Low $\mathbf{\beta^{*}}$ Optics}

Certain physics observables require that the forward detector information is combined with that of the corresponding central detector. In this case the synchronisation of the specific  
forward detector systems with the central detector needs to be considered in the design of the trigger and data acquisition. The distance of up to 250\,m from the forward deFtectors to 
the central detectors requires fast signal transmission and precision clock distribution systems. 
An important impact on the detector design and general layout is given by the machine settings. 
The physics programme outlined in Chapter\ref{sec:introduction} of this report specifies the different LHC beam optics, beam parameters and instantaneous luminosity for the measurement of 
a given physics variable. The requirements for the operation of detectors and movable beam inserts at low and high $\beta^{*}$ are quite different.

The LHC beam intensity setting and instantaneous luminosity for the special runs (high $\beta^{*}$) will be defined by the forward physics community in agreement with the LHC operation group, 
while the integral time for these special runs is subject to negotiation with the LHC scientific management of CERN. 

For high $\beta^{*}$ runs, the integral luminosity per run and the integral beam time per year is much lower with respect to the standard runs, leading to significantly lower instantaneous and 
integral radiation exposure to ionizing and non-ionizing radiation of the dedicated detectors and carriers. However, forward tracking detectors optimized in view of radiation hardness and 
{\bf multi}-track resolution combined with timing detectors synchronized with precision clock distribution systems allow background elimination and vertex separation in the central detectors. 
Such optimized forward detector systems allow higher instantaneous luminosities with the advantage of reaching the physics goals with significantly shorter beam time. 

The forward physics programme at low $\beta^{*}$ in contrary needs to cope with the beam parameters determined by the mainstream LHC physics community, and all detector components to 
be used under these beam conditions are forced to be adopted accordingly. The detector components installed for this purpose can be exposed to very high radiation levels depending on 
the final location of the detector the tunnel or in the central detector.  
In particular, the movable beam inserts need to cope with these machine boundary conditions during insertion under standard run conditions. The design of the beam inserts in view of 
impedance and material budget is one key issue to avoid any impact on the machine stability. To assure the compliance of the beam inserts with the machine requirements, the design and 
production of the beam inserts undergoes strict quality control in close collaboration with the LHC machine safety experts.  As the requirements for movable beam inserts and their corresponding 
detectors differ for the usage in high and low $\beta^{*}$ beams, the following sections describe the detector systems of the different experiments separately for the two main optics settings. 
 {\bf not always specified.}

\input{detectors/alpha_yr.tex}

\section{TOTEM Experiment}
%
%TOTEM and CMS are two independent collaborations working closely together on forward physics with detectors located at IP5 and in the long straight tunnel section within $\pm 220\,$m from IP5.

The TOTEM experiment~\cite{totem-tdr,jinst-totem} is dedicated to
the measurement of the total proton-proton cross-section and to the study of elastic and diffractive scattering. %at high $\beta^{*}$ beam optics.
Two tracking telescopes, T1 and T2, integrated in the CMS detector, cover the pseudo-rapidity region
between 3.1 and 6.5 on both sides of the interaction point. The Roman Pot (RP) stations are located at distances up to $\pm 220\,$m from IP5 to measure the very forward scattered protons at angles of 
the order of microradians. During the LHC Run 1 period (2010--2012), TOTEM performed high $\beta^*$ runs both standalone with T1, T2 and RPs, and combined with the CMS central detector. 
The latter resulted in joined data analysis and common publications. 
As described in the previous Chapters, this common programme with CMS will continue during RunII. 

During LS1 (2013--2014) the TOTEM experiment underwent a consolidation and upgrade programme~\cite{totem-upgrade-proposal,ecr-consolidation,ecr-upgrade,totem-upgrade-tdr} which 
concerned mainly the RP system with the aim to improve the physics capabilities for both high and low $\beta^{*}$ runs. A new RP system layout at $\pm (203\div214)$\,m from IP5 realized during 
LS1 and the future integration of timing detectors in vertical RPs will allow the reach of new physics goals for high $\beta^{*}$ optics. 

The layout of the TOTEM experiment before LS1 can be found in all detail in~\cite{jinst-totem} for both the telescopes (T1,T2) and the RPs. The following section puts the main focus on the new RP layout 
as it was realized during LSl.
Figures~\ref{fig:totem_layout},~\ref{fig:totem_layout_rp} shows the TOTEM experiment with the detectors T1 and T2 embedded in the CMS central detector and the RPs on both sides of CMS after LS1. The following sections 
are based on different documents~\cite{totem-upgrade-proposal,totem-upgrade-tdr,ctpps-tdr}. 

%
\begin{figure}[h]
  \centering
\includegraphics[width=\textwidth]{figs/detector/inelastic-1.png} 
  \caption{The TOTEM forward trackers T1 and T2 embedded in the CMS detector}
  \label{fig:totem_layout}
\end{figure}

\begin{figure}[h]
  \centering
\includegraphics[width=0.9\textwidth]{figs/detector/totem_new_layout_RP.png}  
  \caption{The LHC beam line on one side of interaction point IP5 after LS1: the TOTEM Roman
Pots are installed at distances of 210-220\,m.}
  \label{fig:totem_layout_rp}
\end{figure}

\subsection{Standard TOTEM Detectors Operated during Run-I at High $\beta^{*}$}

\paragraph*{The Telescopes T1 and T2}
%
Figure~\ref{fig:t1+t2} shows the telescopes T1 and T2 and their integration in CMS.
The T1 telescope consists of two arms, on either side of the IP5, fully integrated in the high-$\eta$ cone of the CMS end-cap at a distance between 7.5 and 10.5\,m from the IP. T1 
detects charged particles in the pseudorapidity range 
$3.1 < |\eta| < 4.7$. Each arm is composed of 5 planes of Cathode Strip Chambers, with six chambers per plane~\cite{jinst-totem}. 
The T2 telescope, based on ``Gas Electron Multiplier'' (GEM) technology~\cite{gem_reference}, allows charged track reconstruction in the pseudorapidity range 
$5.3 < |\eta| < 6.5$. Each T2 telescope arm located at $\sim13.5$\,m on either side of IP5 is composed of 20 semi-circular GEM planes - with overlapping regions - interleaved on both 
sides of the beam vacuum chamber to form ten detector planes of full azimuthal coverage~\cite{jinst-totem}. This novel triple GEM detector technology with the combined pad and strip readout 
was optimized to cope with the specific event topology and high radiation load close to the beam tube. In the triple GEM structure, a 3\,mm drift space is followed by two 2\,mm deep charge 
transfer regions (Transfer 1 and Transfer 2) and a 2\,mm charge induction space. Each GEM readout board contains 256 concentric circular strips for the radial coordinate (80\,$\mu$m wide, 
pitch of 400\,$\mu$m) allowing a track resolution of about 100\,$\mu$m, and a matrix of 1560 pads (with varying size from $2\times2\,\rm mm^{2}$ to $7\times7\,\rm mm^{2}$) for azimuthal 
coordinate reconstruction and for the T2 local trigger. The T2 GEM detector is operated with the gas mixture Ar/CO$_{2}$ (70\%/30\%). 

%
\begin{figure}[h]
  \centering
  \includegraphics[width=0.5\textwidth]{figs/detector/T1_20110117_130.jpg} 
  \includegraphics[trim=0mm 55mm 0mm 10mm,clip,width=0.49\textwidth]{figs/detector/t2photo.jpg} 
  \caption{The T1 (left) and T2 (right) telescopes integrated in CMS central detector.}
  \label{fig:t1+t2}
\end{figure}


\paragraph*{Roman Pot System}

The movable beam-pipe insertions called Roman Pots~\cite{jinst-totem} are optimized to detect the leading protons scattered at very small angles. Each RP station is composed of 
two units (near and far) separated by a distance of $\sim 5$\,m, each consisting of two vertical pots and one horizontal pot. On each side of the interaction point IP5, 2 RP stations are installed, 
resulting in a total of 24 single RP detectors, not counting the two new horizontal RPs for timing, added during LS1. Each RP detector is equipped with a stack of 10 edgeless Si strip planes fixed 
in a frame with a high mechanical precision of better than 50\,$\mu$m 
(Figure~\ref{fig:romanpots}, left). The 512 strips with a pitch of 66\,$\mu$m of a single Si-plane are oriented at an angle of $+45^{\circ}$ (u-planes) or $-45^{\circ}$ (v-planes) 
relative to the detector edge facing the beam. Each stack is composed of 5 pairs of u- and v-planes mounted back-to-back and centered inside the RP 
(Figure~\ref{fig:romanpots}, right), that separates the sensors and the associated frontend electronics from the LHC vacuum via a thin window of 150\,$\mu$m thickness. 
The Si detectors with the frontend electronics are operated at $-30^{\circ}$C by means of evaporative cooling. The pressure in the pot is kept between 10\,mbar and 40\,mbar absolute to avoid 
condensation. In case of vacuum problems or increase of the absolute pressure above 50\,mbar absolute, the cooling system is automatically switching to the `warm mode', stabilizing the 
temperature at $+12^{\circ}$C.  To optimize the acceptance for protons scattered at the smallest angles, the TOTEM experiment has developed planar edgeless silicon detectors~\cite{cts_ref1} 
with a Current Terminating Structure (CTS) to reduce the insensitive area at the edge facing the beam down to 50\,$\rm\mu$m 
(Figure~\ref{fig:cts_detectors}, left). The edgeless Si sensors are processed on very high resistivity n-type silicon wafers ($> 10\,\rm k\Omega\,cm$), with a thickness of 300\,$\mu$m. 
The silicon detector hybrid carries the sensor with the 512 strips wire-bonded to the input channels of 4 VFAT readout chips. Beam tests have shown that the full detection efficiency 
is achieved at a distance of only 50\,$\mu$m from the cut edge 
(Figure~\ref{fig:cts_detectors}, right).

%
\begin{figure}[h]
  \centering
  \includegraphics[width=0.8\textwidth]{figs/detector/Fig_RP_draft.png} 
  %\vspace*{5cm}
  \caption{Si detector package composed of 10 Si planes (left). Roman Pot, to
separate the Si detector from the LHC vacuum via a thin window of 150$\mu$m 
thickness (right).
  }
  \label{fig:romanpots}
\end{figure}

%
\begin{figure}[h]
  \centering
\includegraphics[width=0.6\textwidth]{figs/detector/Fig_cts_draft.png} 
%  \includegraphics[width=0.35\textwidth]{figs/detector/} 
  %\vspace*{5cm}
  \caption{(left) Edgeless Si strip sensor with Current Terminating Structure. The
detector reaches full efficiency at 50$\mu$m distance from the cutting edge
(right)}
  \label{fig:cts_detectors}
\end{figure}


\subsection{Detector Upgrade for Vertical Roman Pots}
%
To reach the physics goals at high $\beta^{*}$, TOTEM stand-alone and combined runs of the CMS detector with the TOTEM RPs are envisaged. 
The operations of the RPs during run 1 have shown that the RP carriers and the Si strip detectors worked fully satisfactorily both in stand-alone mode and in combination with the CMS 
{\bf detector}.
%tracker. 

\begin{itemize}

\item
Within the consolidation project performed during LS1, the RPs at 147\,m have been relocated to the 210\,m region upstream of the existing RPs at 220\,m to improve the resolution of this 
proton spectrometer. The Roman Pot unit at 210\,m far was rotated by $8^{\circ}$ around the LHC beam axis 
(Figure~\ref{fig:rp-rotation}) relative to the 220\,m station, to increase the multiple-track resolution of the silicon strip detector system~\cite{totem-upgrade-proposal}. 
Furthermore, all RPs of TOTEM were equipped with new ferrites~\cite{ferrites} of higher Curie temperature as it was requested by the LHC machine committee with the aim to improve the beam vacuum.

%
\begin{figure}[h]
  \centering
  \includegraphics[width=0.9\textwidth]{figs/detector/rp_rotation.jpg} 
  \caption{Drawings of the rotated RP units. The view is directed along the outgoing beam.
  }
  \label{fig:rp-rotation}
\end{figure}


\item
As outlined in the physics chapter, high luminosity runs are needed to reach the integrated luminosity within reasonable beam time for special runs of the machine.
Analysis of special run 1 data in combination with simulations have shown that the integration of timing detectors with a timing resolution of 50\,ps can improve the vertex reconstruction 
significantly up to a pileup of $\mu\sim 0.5$. 

Timing detectors with a resolution of 50\,ps in combination with analogue and digital front-end  electronics components are the main elements of the TOTEM upgrade programme as described 
in detail in~\cite{totem-upgrade-tdr}. 
The pixel size and occupancy of the timing detector sensor and the necessary rate capability of the sensor in combination with the full electronics chain were determined by detailed 
simulation studies. As part of the timing detector infrastructure, a precision clock distribution to synchronize the readout electronics of the timing detectors in the two arms of the $\pm$ 210\,m stations 
will be integrated in the LHC tunnel.
While the timing detector infrastructure will be  already installed during LS1, the detector components -- still under development -- can be integrated, thanks 
to the design of the RPs, in short term technical stops. 


\item
The space available to house the timing detectors in the  Vertical RPs  is limited by the dimensions of the carrier box allowing to stack detectors up to 5\,cm. The 
Cerenkov detectors as proposed~\cite{Albrow-ARX-2012} for movable beam inserts cannot be integrated in the vertical RPs as the radiator bar requires at least 12\,cm. 
However, the new horizontal RPs of the CT-PPS project, installed during LS1 with a cylindrical shape and an internal diameter of 14.1\,cm, can house them. This technology will be 
explained in Section~\ref{sec:cylindricalpot} %on upgrade detectors for low $\beta^{*}$ runs later.

To maintain a low occupancy for each detector channel, its segmentation must be properly tuned.
A simple increase of the granularity reducing the pixel size would lead to an impractical growth of the number of channels, which in turn would reflect on the readout, 
requiring for example the development of custom ASICs.

These considerations led to study a design with pixels of different sizes since the track density due to diffractive events and overlapping background is not uniform as 
can be seen in the RP data recorded during Run 1. The pixel size is defined in view of having the same track occupancy in all pixels.
The simulations to study the occupancy of a single pixel and the minimization of the number of channels required in each detector plane suggested that the minimal number of 
pixels of different sizes needed for a good efficiency at higher luminosity is 10 per plane with areas ranging from a few mm$^2$, for the pixels where the track density is larger, 
to several hundreds of mm$^2$ in the peripheral parts of the detection plane. 
The simulation is explained in detail in~\cite{totem-upgrade-tdr} (Section~4.2).
\end{itemize}


% Pixels of different sizes and the required timing resolution determine the selection of the detector technology:  the choice is to use diamond detectors in order to have to deal with
% a variation of the timing response with the pixel size small enough not to degrade the timing resolution.
% In fact for a diamond detector the pixel size barely affects the time response of the signal due to the extremely high impedance of the material.
\subsubsection*{Diamond Detector as Baseline Technology for Timing Sensor} 
The selection of the detector technology has to take into account the required timing resolution and the variable size of the pixels. The best choice is a diamond sensor, 
where the pixel size minimally affects the time response of the signal due to the extremely high impedance of the material, guaranteeing the same resolution all over the detector plane. 
However the charge released from a diamond sensor is small in absolute terms ($\approx\,18\,000~e$ for a thickness of $500\,{\rm \mu m}$, or $\approx 3\,$fC/MIP), and a low noise amplifier 
is needed to keep the S/N ratio large enough. 
Since the diamond resistivity is very high the main noise source is the first stage of the amplifier. 
It is also easy to implement a pattern with pixels of different sizes by means of a simple metallisation on the diamond crystal. 
The front end electronics design will be then a compromise between speed and low noise.

The number of channels required is 10 per plane and the preamplifier stage has to be located near the detector itself. 
A single plane is a $10\times20\,\rm mm^{2}$ diamond sensor.
A board built with controlled impedance material (Roger) will be the mechanical support of the detectors (glued with the smallest pixel sizes located near the edge closer to the beam), 
and of the preamplifier electronics in order to reduce to the minimum the input capacitance 
(see Figure~\ref{fig:diamond-plane}).
A package of 4 detector planes, with thickness up to 500\,$\mu$m, will fit in a vertical RP. Within
the present state of the art of
diamond substrates it is possible to build detectors
with resolution of the order of 100-150 ps, as the multiple measurements allow to reduce the overall time resolution down to the required $\sim$ 50\,ps.
The readout board will be located as close as possible to the detector . 

%
\begin{figure}[htb!]
 \begin{center}
 \includegraphics[trim=50mm 1mm 60mm 20mm, clip,width=0.6\textwidth]{figs/detector/angle2.pdf}
 \caption{The layout of the board showing the pixel position for one diamond detector plane.}
  \label{fig:diamond-plane}
 \end{center} 
\end{figure}


\subsubsection*{Electronics for Timing Detectors}
\label{sec:Readoutelectronics}
%
Given the small number of electronics channels required for the readout, TOTEM is developing a discrete component amplifiers.
This  single channel preamplifier is made up of two stages, i) the first is a simple CE transimpedance amplifier, with low amplification power and high bandwidth  that allows fine tuning of 
the input impedance (Silicon-Germanium transistors from Infineon are under test). 
The controlled output signal has 50\,$\Omega$ impedance. ii)  The next stage amplifies the signal to an output voltage range of 0-1\,V to match the readout requirements. 
The detector hybrid will contain only the first stage of the amplification chain and the signals are sent through coaxial cables to the second stage amplification board.
The Hybrid is in the secondary vacuum and the cooling is performed passively through the metallic layers of the board itself.

There are two possible ways of adding a time stamp to the recorded protons:  a TDC connected with single or multiple threshold discriminators or a high bandwidth signal sampler. 
The two possibilities considered have slightly different performances:  the first gives a better trigger capability, while the second has a better time resolution.

{\underline {Discriminator and  time-over-threshold measurement with a TDC}}: each pixel is equipped with a wide bandwidth transconductance preamplifier and the output voltage is 
proportional to the input current generated from the collected charge that discharges on the input resistance. 
A single threshold discriminator detects the edge of the signal.
The time walk of a single threshold discriminators, consequence of charge fluctuations, can be corrected  measuring the time over threshold for each signal. 
In this case the signal rise time is limited by the bandwidth and with the present electronics is possible to obtain rise time down to $\sim180\,\rm ps$.
The criticality of this approach is that for a MIP the signal to noise ratio is lower than 2.
A way to improve the S/N is either to add coherently with one preamplifier the signal produced in two (or more) diamond planes connected in parallel or to increase the input 
resistance of the amplifier as discussed in~\cite{osipenko2013comparison}. 
However the understanding of both solutions requires a certain amount of simulations and tests.
%
 \begin{figure}
 \begin{center}
 \includegraphics[width=.5\linewidth]{figs/detector/DSC4135-10cm-300DPI.jpg}
 \caption{The board with the SAMPIC chip, developed in Saclay, used for the first tests.}
  \label{fig:sampic-board}
 \end{center} 
\end{figure}

The NINO chip~\cite{anghinolfi2004nino} provides this possibility, the output signal length being proportional to the time over threshold of the input analog signal. 
The maximum acquisition rate of this device is around 30\,MHz which in turn implies an average rate for each pixel of less than 10\,MHz, well below the maximum rate expected in the experiment.
The front-end board for one plane will have 10 LVDS output signals each one providing both the pixel information of time of arrival with the leading edge and the charge released with the signal length.

{\underline {Digital sampling}}: the signal from each pixel is integrated and then sampled with a high bandwidth signal sampler.
To extract the timing information from the output of a preamplifier with a known transfer function, an appropriate algorithm reconstructs the original signal.


The sampling can be performed with the SAMPIC chip developed in Saclay~\cite{GrabasPhD}. 
The chip has 16 input channels with a  sampling rate up to 10\,Gs/s which provides a good signal reconstruction for signals with a rise
time of 1-3\,ns 
(see Figure~\ref{fig:sampic-board}).
This gives some margin to increase the signal-to-noise ratio for the
preamplifier.

For each channel a circular buffer of capacitors continuously samples the input signal.
Digitization  of the buffer using a 11 bit Wilkinson ADC starts either  when an external trigger is provided or when the input signals goes above a programmable threshold 
(see Figure~\ref{fig:SAMPIC_Principle} for a diagram of the chip).
%
\begin{figure}[htb]
 \begin{center}
  \includegraphics[width=.7\linewidth]{figs/detector/SAMPIC_Principle.pdf}
  \caption{Inside the SAMPIC, the input signal is continuously sampled in a ring analog buffer. In internal trigger mode, the signal is compared to a programmable threshold to stop the sampling 
   and start the ADC conversion.}
  \label{fig:SAMPIC_Principle}
 \end{center} 
\end{figure}

A future version of the chip will allow a minimum 50\,ns dead time on each independent  channel by using  a faster interleaved readout between two or four channels and a function to control the 
internal trigger, for instance start conversion only when the internal trigger fires in coincidence with the bunch crossing, and the possibility of a fast read-out of the internal trigger time-stamp 
to be complemented with a more precise timing information after the digital analysis of the sampled signal will be completed.

The SAMPIC with a CSA preamplifier has been tested with a pair of ``Ultra-Fast'' Silicon detectors~\cite{cartiglia2013performance}.
Figure~\ref{fig:Si_CSA_6-4_CC} shows the time difference measured between the two detectors pulsed with the same laser via an optical splitter and using an off-line algorithm. 
The resolution achieved on the timing difference is of $\sim 40 \,$ps, which indicates a resolution of $\sim 30\,$ps for a single measurement. More studies will follow with diamond detectors in a real 
test beam or cosmic rays.

%
\begin{figure}[htb!]
 \begin{center}
  \includegraphics[width=.7\linewidth]{figs/detector/Si_CSA_6-4_CC}
  \caption{Distribution of the time difference between two Ultra-Fast Silicon detectors pulsed with the same laser and read with fast CSA and SAMPIC, using an advanced off-line algorithm. } 
  \label{fig:Si_CSA_6-4_CC}
 \end{center} 
\end{figure}
%

{\underline {Preliminary Tests:}}
Two diamond detectors, $0.5\times0.5\,\rm mm^{2}$ in size and 500\,$\mu$m in thickness, have been purchased from Cividec Instrumentation~\cite{cividec} together with state of the art CSA and wide-band 
amplifiers with specs optimized to  our request, and assembled in a telescope 
(Figure~\ref{fig:DiamondDet}) for measurements with particles on a test beam (Figure~\ref{fig:DiamondSig}).
Moreover new transimpedance preamplifiers have been developed in house in order to study and optimise the input impedance of the circuits.
Three beam test have been performed in PSI and Cern PS, with different configurations. The detectors where connected to the preamplifiers with SMA connectors. The input capacitance, of about 0.5\,pF from 
the detector, was dominated by the connectors and the cables (5-10 pF). The rise time of the signals is strongly affected by this parameter and therefore a reduction in performance is expected. The resolution obtained 
is around 190 ps, well in line with the expected value, and a dramatic improvement is expected with a design of the hybrid that removes the connector. 
The final step is therefore to design and bring to a test-beam a hybrid with first-stage preamplifiers bonded as close as possible to the detector, in order to keep the capacitance below
$\sim 1$\,pF. A similar design has already been used successfully elsewhere~\cite{Bousonville:2009}. Construction of the new hybrid has already started.


{\underline {Other Technical Considerations:}}
A cooling system will be provided for the electronics only, since the diamond detectors do not dissipate any power from the polarization power supply.

All the electronics that need to be as close as possible to the actual detector and that makes use of FPGAs (as the control/transmission board for the SAMPIC or, in alternative, the TDC board) can operate 
only in regions with reasonable radiation levels.
Studies performed on Altera Cyclone FPGA with ion and neutron beams  show that even in the surrounding area of the beam pipe we could expect for high luminosity runs a SEU (single event upset) rate of 
1 every 3 hours, which is already orders of magnitude higher than what was experienced in the special high beta optics runs. 
For this reason space close to the Roman Pot station located in the floor of the tunnel will be available  to keep the electronics as far possible from the beam pipes. 
In case of SEU a Resync request will be needed only for  the TDC board.

\begin{figure}[htb!]
 \begin{center}
\includegraphics[width=.48\linewidth]{figs/detector/DiamondDetector_low-small.pdf}  
\includegraphics[width=.48\linewidth]{figs/detector/D-DetectorInBox-small.pdf}
  \caption{Prototype of the diamond detector from Cividec Instrumentation (left) and the assembly of  the test  telescope (right).}
  \label{fig:DiamondDet}
 \end{center} 
\end{figure}
%
\begin{figure}[htb!]
 \begin{center}
  \includegraphics[width=.7\linewidth]{figs/detector/DiamondEVTDisplayTDR.png}
  \caption{NEW? 
  Signals of two diamond detectors read with a fast Charge Sensitive Amplifier in a test beam measurement with 12\,GeV ${\pi}^-$.}
  \label{fig:DiamondSig}
 \end{center} 
\end{figure}

TDCs  with a time resolution of $\sim$\,10\,ps inside an FPGA are in an advanced stage of development by TOTEM and under evaluation. 
The time reconstruction algorithm measures the  crossing time for a single threshold and the time over threshold and a correction matrix. 
In case we will use the SAMPIC chip, the data have to be fitted in a simple FPGA board.
The advantage of using on board FPGAs is that the Trigger and DAQ information will be formatted on the same board.
The event is formatted for DAQ with a header, a start of frame patterns and counters, the list of TOA (Time Of Arrival) and TOT (Time Over Threshold) for each fired pixel, and a footer. 
The information is transmitted without on-line corrections.

The Trigger algorithm instead will perform an on-line rejection based on the number of tracks (see~\cite{totem-upgrade-tdr}, Section~4.2.2). 
In order to filter out noisy channels that could contaminate the time measurement a trigger signal (a track road) is generated only if the signals from aligned pixels from adjacent planes satisfy a 
majority-AND condition. 
Track counting is done locally and, if the event is accepted, the time of arrival is formatted into 4 words and sent to the central trigger unit (TOTEM LONEG board). 

\subsubsection*{Clock Distribution for Timing Detectors at $\pm\,$220\,m from IP5}
%
The challenge of combining measurements with picosecond range precision for Timing signals generated in locations separated by large distances (order of 220\,m) requires a clock distribution system 
capable of the highest precision and of the utmost time stability. 

The following pages aim at describing the Clock Distribution system for the TOTEM Timing Upgrade.
The system is adapted from the \textit{Universal Picosecond Timing System}~\cite{Bousonville:2009}, developed for FAIR (Facility for Antiproton and Ion Research), the new, unique international 
accelerator facility for research with antiprotons and ions presently under construction at GSI (D), where a Bunch phase Timing System (BuTiS) based on this 
concept has been implemented~\cite{Moritz:2011zz}.

The optical clock distribution network will use a Dense Wavelength Division Multiplex (DWDM) technique that makes it possible to transmit multiple signals of different wave-lengths 
over a common single mode fibers. This will allow to use standard telecommunication modules compliant to ITU (International Telecommunications Union) international standards.

The experiment requires two very stable clocks for the precise timing reference of the measurement and the bunch identification. 
These reference clock signals are sent from the counting room to a set of receivers positioned near the timing detectors in various location of the LHC tunnel on both sides of IP5. 
A third signal added  on the same optical fiber will be simply reflected back to be used to continuously measure the time delay of each optical transmission line: these delay measurements 
are necessary to correct the time information generated at the detector location for fiber delay variations (thermal and mechanical instabilities). 

The system can be logically subdivided in four major blocks: the Transmission Unit, the Distribution Unit, the Measurement Unit and the Receiving Unit. 
One Receiving Unit must be installed very near each Roman Pot location, the Transmission, Distribution and Measurement Units will be located in the TOTEM racks in the IP5 counting room.
A block diagram of the entire system is reproduced in Figure~\ref{fig:CD-fig1-fullpage}. 
%
\begin{figure}[ht!]
    \begin{center}
    \includegraphics[width=0.95\textwidth]{figs/detector/distribution-TU_fig2}
    \caption{The clock distribution system.}
    \label{fig:CD-fig1-fullpage}
    \end{center}
\end{figure}

Measurements performed with the prototype of the ``BuTiS'' system show that the influence of the transmission system on the signal jitter, is of the order of 0.4\,ps~\cite{Moritz:2011zz}, mainly 
dependent on the quality of the clock source signal, the noise added by the optical components and the bandwidth of the transmission system itself. 
Using a transmission system based on this concept, the total jitter of the TOTEM clock transmission system will also be due mainly to the  inherent jitter of clock sources and the end user electronics. 


\begin{itemize}
\item Transmission unit\\
%
The Transmission Unit  optically modulates  the two reference clocks in signals with different wavelength  $\lambda_1$ and $\lambda_2$.
Via DWDM these optical signal are multiplexed into a single fiber 
and re-transmitted at a specific wavelength using a 1\,550\,nm band laser to the Distribution Unit. 
The signal is amplified with an erbium-doped fiber amplifier (EDFA) to compensate the attenuation due to further splitting and the multiplexers. 

A Thorlabs PRO8000~\cite{thorlabs} 
platform has been chosen to generate the two DWDM wavelengths on channels ITU 32 and ITU 34.
 This complete platform is designed to operate and control electrical and optical modules for telecommunication testing and application developments from a broad family of interchangeable modular 
 devices and can be controlled by an external computer using industrial control protocols.
The modulation of the optical signals is performed by two military grade Mach-Zehnder modulators with a 20\,GHz bandwidth.
This unit can be rack mounted and is suitable for use in the experiment control room harsh environment. 

\item Distribution Unit\\
%
The DWDM optical signal, as generated by the Transmission Unit, needs to be split in order to be transmitted to the four Receiving Units.
Moreover a third DWDM modulated optical signal of wavelength $\lambda_M$ is needed to measure the transmission delays over each fiber and is added to the other two clock signals. 
 
The JDSU~\cite{jdsu} Multiple Application Platform (MAP-200) has been chosen for the Distribution Unit optical amplification, optical signal splitting and switching. 
This platform is a highly configurable, scalable and industrially controlled system that can host several optical modules with a wide range of functions.
The EDFA amplifier developed for this platform will be used for the signal optical amplification.

\item Measurement Unit\\
%
The signals' delays are measured in this unit.  
A reference signal is generated, optically modulated using the wavelength $\lambda_M$ and sent via an optical switch to every Receiving Unit and to a reflector, which will be used for calibration.

Add/drop multiplexers combine this reference signal to each of  the  4 DWDM optical signals generated in the Transmission Unit and split in the Distribution Unit. 
The multiplexed signal, that now contains the three modulated optical wavelengths: $\lambda_1$, $\lambda_2$ and $\lambda_M$, is transmitted to the Receiving Units located in the tunnel at $\pm220$m and $\pm210$m.

The  $\lambda_M$ optical reference signal once at  the Receiving Unit is reflected back to the Measurement Unit, where the optical add/drop multiplexer separates the $\lambda_M$ optical signal 
coming back from the RUs and pass it back to the optical switch.  
 A ``circulator'', placed between the DWDM modulator and the switch, distributes the reflected signals to a measurement instrument without interrupting the transmission from the generation module to the switch. 
A phase comparison of the reflected signal with the reference one is performed, using a vector network analyzer. 
The phase differences obtained by this measurement determine the delay of each clock signal distribution channel.

As for the Transmission Unit, a Thorlab PRO8000 module, and the same Mach-Zender modulator, will be used.  
The DWDM wavelengths proper of channel ITU 36, will be used to modulate the reference signal.

\item Receiving Unit\\
%
The Receiving Unit separates the multi-wavelength optical signal at the RP stations into individual signals.

The signal from the single mode fiber (SMF) encounters first a  Bragg grating (FBG) DWDM reflector and reflects back the signal component of $\lambda_M$ wavelength. 
The other components of the signal are routed to a DWDM demultiplexer that separates the two wavelengths, $\lambda_1$ and $\lambda_2$, and outputs them on separate fibers for conversion to 
electrical signals and delivered to the front end electronics and DAQ cards eventually.

This unit should be located as close as possible to every Roman Pot location.
A temperature stabilization of this unit, depending on the temperature characterization of the installation point in the tunnel, may be needed to reduce the long term shift of the measured delay. 
\end{itemize}


\section{CMS-TOTEM Proton Spectrometer (CT-PPS)}

A new collaboration between CMS and 
TOTEM was created to develop the 
CMS-TOTEM Precision Proton Spectrometer~\cite{ctpps-tdr} related to the physics goals reachable with low $\beta^{*}$ optics (standard LHC settings). The baseline  carriers of 
this spectrometer are the newly developed low-impedance RPs integrated in the beam line at $\pm (203\div214)$\,m from IP5, designed to host future pixel and picosecond-timing detectors. 
To optimize the beam quality and to protect the LHC magnets near the RPs against collision debris, new collimators were installed upstream (TCL4) and downstream (TCL6) of the RPs during LS1. 
The TCL4 collimators were installed in the former locations of the RP147 stations, and TCL6 was installed between the most downstream unit of RP220 and the supra-conducting magnet Q6.
 Comprehensive simulation studies were performed and it could be shown that optimized collimator settings can result in a satisfactory machine protection without limitation of the physics goals. 
 Additional beam loss monitors (BLMs) were installed in that region to monitor beam losses caused by RP and TCL6 insertions in that critical region.  
The installed spectrometer will consist of a total of 26 RPs (7 horizontal and 6 vertical RPs on each side of IP5) that can be inserted selectively.


%\subsubsection{Movable Beam Inserts, Collimators and Detectors for Low $\beta^{*}$} 
%
Within the CT-PPS collaboration new movable beam inserts, tracking and timing detectors for the low $\beta^{*}$ forward physics were developed for the LHC straight line beam region of $\pm$\,210\,m from the interaction point IP5.
The requirements on beam inserts and detectors operated at low $\beta^{*}$ are quite different from those at high $\beta^{*}$, as already outlined in XXX. 
The underlying strategy foresees to integrate where possible the 
newly developed  detectors in existing carrier systems of TOTEM and the use of existing infrastructure in the LHC tunnel. This concept lead to an inter weaved project of the TOTEM consolidation and upgrade program with the CT-PPS project. 
Timing detectors with a resolution better than 10\,ps are required to achieve  the necessary vertex separation in the CMS central detector with a O(mm) precision. The double hit probability per bunch crossing and the acceptable single proton rate of a 
single timing cell  determine the pixel size.   
The detector systems with this time resolution and pixels size, combined with the high rate requirements, represent the forefront of present detector developments. With Cerenkov detectors, that can be integrated in the newly developed Roman Pots,  
the time resolutions in the range of 10\,ps could already be achieved in test beams, however the high material budget and limited pixel size of this technology might turn out to be a limiting factor in the final operation under LHC conditions. 
Therefore R\&D of different solid state detector have started to obtain the required time resolution with a lower material budget and smaller pixel cell size.
The edgeless Si strip tracking detectors of TOTEM can not be used for the low $\beta^{*}$ operation due to the intrinsic limited  multi hit resolution. New slim edge radiation hard  pixel detectors that cope with the required space resolution and 
optimized for the use in movable beam inserts are under development. 

The upgrade of the present Roman Pots and the development of new cylindrical Roman Pots was mandatory for the ambitious goal to insert the detectors under standard LHC conditions close to the beam. 
At this point it is emphasized that alternative beam inserts like the movable beam pipe with low impedance (Hamburg Beam Pipe) have been studied for many years and are still under development~\cite{hamburg-beampipe}. The movable beam pipe concept, primarily 
developed for locations at LHC where the operation of horizontal Roman Pots is almost impossible due to space constraints of the LHC beam line, was as well proposed as alternative in that locations, where the Roman Pots 
are at present integrated in the beam line of $\pm$220\,m from IP5. However, till today  was neither reached a final design nor the construction of a full size prototype, that complies with all requirements imposed on a beam insert for LHC. The possible usage of 
these type of beam inserts requires further R\&D and the successful construction and test of a full size prototype.

In the absence of feasible alternatives to the concept of the Roman Pot at the time of LS1, the TOTEM collaboration decided for time and cost reasons to study and develop in close collaboration with the 
LHC Beams Impedance and engineering groups, the low 
impedance Roman Pot concepts, based on the experience made during three years of operation during run1 of LHC. These developments lead over a prototype phase, including mechanical \& vacuum tests  and  RF measurements simulating the EM radiation field of 
the LHC beam close to the Roman Pot to a final design, that was approved for serial production. Even though the simulation and lab test have shown significant improvement of all critical parameters that determine the successful and safe operation of these 
beam inserts,  a final prove of the expected performance can only be made under realistic conditions of LHC. In this sense the newly installed Roman Pots within the CT-PPS project can be considered as R\&D for new beam inserts designs. 
     
Test insertions of horizontal Roman Pots by TOTEM during run 1 have shown, that the generated secondary particle production rate impinging on the magnets downstream of the 220\,m far Roman Pot stations can exceed the acceptable level. 
For that reason a new collimator system (TCL4 and TCL6) was proposed for IP1 and IP5, and installed during LS1~\cite{ecrcollim}. 
Figures~\ref{fig:layout} and~\ref{fig:layoutphoto} show the beamline in Sector 4-5 with the RPs installed.
 
 
 
%\iffalse 
 
% \subsubsection{The Roman Pot System and Collimator in the 200\,m Region of IP5}
%The TOTEM consolidation and CT-PPS project combines the relocated Roman Pots (box shape) to house new pixel tracking detectors (RP210 near-horizontal and RP210 far-horizontal) with the
%newly fabricated cylindrical Roman Pots to house timing detectors. The requirements for both the beam inserts and the detectors are very different for the operation at standard LHC conditions (low beta*)   
% Within the TOTEM R\&D project a cylindrical RP 
%has been newly designed to house timing detectors and was optimized in view of material budget and RF interaction with the LHC beam. Furthermore, 
%the horizontal RP210 destined to house the new tracking pixel detectors,  have been optimized to reduce the RF interaction with LHC by keeping the original box design of the standard TOTEM RP. 
%        
%TCL4 and TCL6 collimators have been installed~\cite{ecrcollim} in front of the Q4 and Q6 quadrupoles, respectively.
%Figure~\ref{fig:layoutphoto} shows the beamline in Sector 4-5 with the RPs installed.

%\fi
 
\begin{figure}[h!]
\begin{center}
\includegraphics[width=0.95\linewidth]{figs/detector/layout.png}
%\vspace*{5cm}
\caption{The layout of the beam line in the 200 m region after LS1}
\label{fig:layout}
\end{center}
\end{figure}

\begin{figure}[h!]
\begin{center}
\includegraphics[width=0.95\linewidth]{figs/detector/45_all_installed.jpg}
%\vspace*{5cm}
\caption{The beamline in Sector 4-5 with the RPs installed}
\label{fig:layoutphoto}
\end{center}
\end{figure}



\subsection{Development of Low-Impedance Roman Pots}
\label{sec:cylindricalpot}

The new RPs installed between the existing units 
220-N and 220-F are intended to host timing detectors. Hence their design was
subject to the following main requirements:
\begin{enumerate}
\item Among several potential detector technologies for the timing
measurements (see Section~\ref{sec:timing_cherenkov}), \v{C}erenkov counters~\cite{Albrow-ARX-2012,atlas_upgrade}
are already at well advanced development stage.
For the full timing resolution of $\sim\,15$\,ps a total 
length of 24\,cm of quartz is needed. Distributing this length over the two 
new pots requires each pot to accomodate two slabs of 6\,cm length, too big
for the space provided by the traditional TOTEM pots.
If at a later stage thinner timing detectors (e.g. diamond detectors) become 
available, tracking and timing functionality may be combined in the same pots,
reducing the number of pots to be inserted.
\item The RPs housing the timing detectors will have to operate in  
high luminosity running scenarios. They will have to approach very intense 
beams to the same distance as the tracking RPs, i.e. down to about a mm from
the centre. At that distance beam-coupling impedance effects, machine vacuum
compatibility in terms of outgassing, and particle 
shower development have to be taken into account in the geometrical design and
in the choice of materials (Section~\ref{sec:beamenvironment2012}).
\end{enumerate}
%
\begin{figure}[ht!]
\begin{center}
\includegraphics[height=5cm]{figs/detector/cylindrical_pot.jpg}
\includegraphics[height=5cm]{figs/detector/cylindrical_pot2.jpg}
\includegraphics[height=5cm]{figs/detector/cylind_photo.jpg}
\caption{Top: drawings of the cylindrical detector housing for the new RPs designed 
to accomodate timing detectors. Bottom: the manufactured pots.
}
\label{fig:cylindricalpot}
\end{center}
\end{figure}
%
\begin{figure}[h!]
\centering
\includegraphics[width=0.8\linewidth]{figs/detector/production_drawing_cylindrical_new.jpg}
%%\vspace*{5cm}
\caption{Dimensions of the cylindrical RP.}
\label{fig:cylindricalpot_dimensions}
\end{figure}
%
After considering various options and after an iterative optimisation, the 
following design has been adopted for the new RPs 
(Figures~\ref{fig:cylindricalpot} and~\ref{fig:cylindricalpot_dimensions})~\cite{JBEDMS}.
The volume housing the detectors will have a cylindrical rather than rectangular
box shape. This choice provides the necessary space for all potential 
technologies of timing detectors and at the same time reduces the beam 
coupling impedance by minimising resonant cavities.
The ferrite in this design will be integrated in the 
(stationary) flange rather than mounted on the moving detector housing. It will have
a ring geometry (inner diameter = 150\,mm, radial 
width = 15\,mm, thickness = 5\,mm).
Furthermore, all vacuum-side surfaces of the RP stations are foreseen to
receive a $2\,\mu$m thick Non-Evaporative Getter (NEG) coating.


\subsubsection{The Mechanical Tests of New Roman Pot Cylinders}
The new cylindrical Roman Pots with the thin window of 300\,$\mu$m thickness have been produced (see Figure~\ref{fig:cylindricalpot}) in a collaboration of CERN with industries. 
After the production of the first prototype in fall 2013 a series of test have been performed at CERN in collaboration with different support groups, 
to approve the compatibility  of this new RP design with the LHC requirements.
The deflection of the thin window was measured as function of the applied air overpressure
simulating the possible pressure difference seen by the RP when the LHC beam tube is under vacuum and the inner side of the RP is under atmospheric pressure.
Such pressure difference will arrive during the installation of the detector components or a failure of the vacuum system and a leak of the 
feedthrough integrated in the flange separating the atmosphere from the inner side of the RP~\cite{edms_rpwind}.  
Furthermore the He transmission was measured in a special setup and the compatibility of this design with the LHC leak rate requirements was shown~\cite{edms_rpleak}.
 


\subsubsection{The RF Shield for the Box-Shaped Horizontal Roman Pots}
\label{sec:rfshield}
Given that the existing horizontal pots housing tracking detectors will have to 
cope with the same high luminosity conditions as the new timing RPs, some 
adaptations will be made:
\begin{itemize}
\item To reach the same impedance reduction as for the new cylindrical pots 
(see Section~\ref{sec:impedance}),
the rectangular detector boxes will be successively 
equipped with 1\,mm thick cylindrical 
copper RF shields (Figure~\ref{fig:cylindricalshield}). Holes in the shield allow 
for the gas flow
necessary to establish a vacuum equilibrium inside and outside the shield.
The number and dimensions of these holes have been defined in cooperation with the 
LHC vacuum group: In the lateral, cylindrical wall there are 3 rows of 15 circular 
holes each with a diameter of 1\,cm; the wall facing the beam has 8
slits of $3 \times 12 \rm mm^{2}$ with rounded corners (2\,mm radius).
The shield is retracted by 30\,mm from the box window facing the beam, in 
order not to intercept any signal protons with the shield material. In the first
step, during LS1, the horizontal pots of the RP210 station will 
receive the RF shields, in order to gain experience without touching the RP220
station.
\item 
The horizontal RP210 stations will be equipped with new vacuum bellows and modified flanges that allow to integrate 
the same ferrite geometry as used in the new RPs. 
The ferrites of the vertical RPs of the RP210 stations will be exchanged with the new TT2 material as in the RP220 stations.
\end{itemize}
%
\begin{figure}[h!]
\begin{center}
\includegraphics[height=4.6cm]{figs/detector/cylindricalshield1.jpg}
\includegraphics[height=4.6cm]{figs/detector/cylindricalshield2.jpg}
\includegraphics[height=4.6cm]{figs/detector/cylindricalshield3.jpg}
\includegraphics[width=6cm]{figs/detector/shielded_photo.jpg}
\caption{Top: Drawings of the cylindrical RF shield for the box-shaped horizontal RPs. Bottom: the manufactured shield.}
\label{fig:cylindricalshield}
\end{center}
\end{figure}
%

\subsubsection{Interaction of the Roman Pot with the Beam Environment}
\label{sec:beamenvironment2012}
In October and November 2012 several test insertions of the RPs in 
normal high-luminosity fills at $\sqrt{s}=8\,$TeV with $\beta^{*}=0.6\,$m were 
performed. While the vertical pots had no problems to reach the target 
distance of 12\,$\,\sigma$ from the beam centre, 
the horizontal pots encountered a very intense collision 
debris halo, and repeatedly the beam was dumped by 
showers hitting the Beam Loss Monitors at a pot position of about 30\,$\sigma$.
Separating the beams in IP5 finally reduced the luminosity -- hence the debris
halo -- by a factor 22.7, enabling the approach to the horizontal target distance
of 14$\,\sigma = 1.6\,$mm from the beam containing 1368 bunches of -- at 
RP insertion time --
$1.1\times10^{11}$ protons or a total charge of $1.45\times10^{14}$ protons. 
The beam profiles (Figure~\ref{fig:beamprofiles}) 
measured during these insertions can be used to benchmark shower simulations 
(Section~\ref{sec:showerMC}).
The first lesson for the upgrade from this exercise is that 
a horizontal RP approach to physics-relevant positions of $10\div15\,\sigma$
will require to absorb the showers produced by the RPs in order to protect the
quadrupole Q6. The solution is the addition of the new collimators
TCL6 between the RR220 station and Q6 (see Section~\ref{sec:collimation}).

%
\begin{figure}[h!]
\begin{center}
\includegraphics[height=5.7cm]{figs/detector/profile_vertical.pdf}
\includegraphics[height=5.4cm]{figs/detector/rate_profile_recuperated.pdf}
%%\vspace*{5cm}
\caption{Left: vertical beam profile measured via the trigger rates in the 
detectors of the top and bottom pots of Sector 56, 220-N. Right: horizontal beam profile
measured in Sector 45, 220-N; the luminosity reduction by beam separation has been 
corrected for. The reconstructed curve is the result of a convolution fit 
discussed in~\cite{frici_note}.
}
\label{fig:beamprofiles}
\end{center}
\end{figure}
%
While the horizontal pots were stationary at 14$\,\sigma$ from the beam centre,
i.e. for about 30 minutes, the temperature sensors on the detector hybrid 
boards in those RPs registered a temperature increase by about 4$^{\circ}$C, 
despite the active cooling of the detector packages. This effect is explained
by impedance heating of the ferrite collar mounted around the box-shaped 
housing on the beam vacuum side. A direct temperature measurement 
near the ferrite was not available, but given the long thermal conduction 
path from
the heat source to the detector package, and the absence of convection inside
the pot due to the secondary vacuum, the temperature of the ferrites may have
reached values well above 100$^{\circ}$C, the Curie temperature of the ferrites
(material 4S60 from Ferroxcube) above which they are ineffective.
Another piece of evidence for substantial heating of the ferrites was given by
the vacuum deterioration observed after the very close insertion of the 
horizontal RPs. First laboratory tests have shown that the ferrite material 
installed around the pots shows substantial outgassing at high temperatures.

Triggered by the problems and observations described above, a programme of 
simulations, extended laboratory tests, and design optimisations
was defined; it is discussed in the following section.

\subsubsection{Impedance}
\label{sec:impedance}
%
{\bf check consistency as it has been reduced....}

As mentioned in the previous section, during a RP insertion to 1.6\,mm 
from a high-intensity beam (1368 bunches of $1.1\times10^{11}$ protons) a 
temperature increase was observed on the detector hybrid boards. This 
effect can probably be attributed to impedance heating. It is 
hypothesised that the 4S60 ferrite mounted around the RP box reached a temperature above
100$^{\circ}$C, the Curie temperature, which resulted in the loss of ferrite 
effectiveness and hence even stronger heating by the now non-damped cavity resonance 
near 550\,MHz~\cite{oldrfnote}. Note, however, that no other impedance effects were 
observed, in particular, no beam instabilities.

The aim of the work presented here~\cite{nicolaminafra} is the optimisation of the RP design to minimise the 
beam-coupling impedance, in particular at very close distances to the beam, in view of
more regular and extended RP insertions in the future.

The impedance seen by a beam of particles has contributions from the shape of the vacuum chamber (geometrical impedance) and from the finite conductivity of the material used for its construction. 
The remainder of this section focusses on the dominant geometrical contribution of three RP designs: the standard box-shaped RP, the new cylindrical RP, and the
improved box-shaped RP with shield (introduced in Section~\ref{sec:rfshield}).

The study was performed by simulating the passage of a charge distribution (source charge) through a cavity, in this case through a RP, and computing the wake field felt by a longitudinally or transversely displaced second charge (test charge).
The potential felt by the test charge is then used to compute the longitudinal or transverse impedance using Fourier Transforms.

Three impedance effects have to be addressed:
\begin{itemize}
\item \textbf{Beam-induced heating}, i.e. the transfer of power from the beam to the 
lossy wall of a cavity, is determined by the frequency-dependent real part of the 
longitudinal impedance in conjunction with the power spectrum of the beam.

%:
%\begin{equation}
%P_{\rm loss} = 2 \, I^2 \sum_{p=0}^{\infty} \emph{PS} (p M\rq{} f_{\rm rev}) \Re [Z_{\rm long} (p \, M\rq{} \, f_{\rm rev})] \: ,
%\label{eqn:ploss}
%\end{equation}
%where
%\begin{itemize}
%	\item $\emph{PS}(f)$ is the power spectrum;
%	\item $f_{\rm rev}$ is the revolution frequency, 11.245\,kHz for the LHC;
%	\item $M\rq{}$ is the number of buckets, 1782 for the LHC with a bunch spacing of 50\,ns;
%	\item $I = M e N_B f_{\rm rev}$ is the beam current, with $M$ number of bunches, $e$ charge of the proton, $N_B$ number of protons per bunch;
%	\item $Z_{\rm long}$ is the longitudinal impedance.
%\end{itemize}
The main contribution to the heating comes from resonances below 1.5\,GHz; at higher
frequencies the beam power spectrum is attenuated by more than $\sim30$\,dB relative to its value at $f = 0$~\cite{baudrenghien2011lhc}.
For all power calculations a current of 0.6~A (corresponding to $M$=2808 and $N_B$= 1.2 $\cdot$ 10$^{11}$ protons) was used.
\item \textbf{Longitudinal instabilities} are related to the effective longitudinal 
impedance.
The effective impedance is the impedance actually felt by the beam: it is given by the impedance convolved with a
weighting function $\sigma(f)$ which is determined by the bunch profile.
%:
%\begin{equation}
%\label{efflongdef}
%	Z^{\rm eff} =\frac{\sum\limits_{f} Z(f) \sigma(f)}{\sum\limits_{f} \sigma(f)}
%\end{equation}
%
A conservative estimation of the effective longitudinal 
impedance is the slope of the imaginary part of the longitudinal impedance
at low frequencies $Z_{\rm long}^0/n$
%:
%\begin{equation}
%\label{efflong}
%	\Im Z_{\rm long}^0/n = \lim_{f \to 0}  \, f_{\rm rev} \,\frac{ 
%{\rm d} \Im Z_{\rm long}}{{\rm d}f}
%\end{equation}
where $n=f/f_{\rm rev}$ is the harmonic number.
It is possible to show~\cite{nicolaminafra} that
$\Im Z_{\rm long}^0/n < (\Im Z_{\rm long}/n)^{\rm eff}$.

The simulated value for $\Im Z^{0}_{\rm long}/n$ will be compared with the measured value for $ (\Im Z_{\rm long}/n)^{\rm eff}_{\rm LHC} = \rm 90\,m\Omega$~\cite{Chapochnikova}.
\item \textbf{Transverse instabilities} have, analogously, their origin in the 
low-frequency behaviour of the transverse impedance. Following the same approach for the effective transverse 
impedance, it is possible to compute the \emph{driving} (or \emph{dipolar}) impedance and relate it to the transverse impedance~\cite{EMetral}, $\Im Z_{\rm t}^{\rm driving}$.

%:
%\begin{equation}
%\label{efftrans}
%\Im Z_{\rm t}^{\rm driving} = \frac{\partial \Im Z_{\rm t}}{\partial t_{\rm source}} 
%\end{equation}
%where $t = x, y$ and $t_{\rm source}$ represents a small transverse displacement of the source charge, which creates
%the wake field, from the nominal position.
%The value is usually constant at low frequency ($< 500$\,MHz).
A normalisation with
the ratio of the beta function value at the equipment under study, 
$\beta_t$, and the 
average over the ring, $\langle\beta_t\rangle = 70\,$m, facilitates the 
comparison with other equipments at different positions in the 
machine:
\begin{equation}
\label{efftransnorm}
\overline{\Im Z_{\rm t}^{\rm driving}} = \Im Z_{\rm t}^{\rm driving} \frac{\beta_t}{\langle\beta_t\rangle} 
\end{equation}
The new RP will be horizontal ($t=x$); moreover, among all the RPs the highest value (worst case) of $\beta_{x} = 98\,$m is reached at the unit 210-N. 
This value can be compared with 25 $\rm M\Omega /m$, a conservative value of the value expected for the full machine~\cite{EMetralTransMeas}.
\end{itemize}

For the new cylindrical pots, simulation results indicate that no low frequency resonances ($<~1.4\,$GHz) are present if the gap between the detector housing and the flange is 
completely closed, which of course would prevent any RP movement.
Mechanical constraints require at least 2.5\,mm gap between the housing and the flange.
With this gap a resonance at 470\,MHz appears,% as shown in Figure~\ref{fig:CylWOF_25mm}; 
its impedance, however, is smaller than for the standard box-shaped RP.
%
%\begin{figure}[h!]
%\centering
%\includegraphics[height=4.5cm]{figs/detector/CylWOF_25mm.jpg}
%%\vspace*{5cm}
%\caption{Simulated $\Re [Z_{\rm long}]$ of the cylindrical RP without ferrite. The resonance at 470\,MHz is due to the cavity between the flange and the detector housing. 
%The darkened part of the graph has negligible impact on the heating due to the 
%strongly attenuated LHC power spectrum at such high frequencies.}
%\label{fig:CylWOF_25mm}
%\end{figure}
The position and the dimensions of the ferrite has been optimised through various iterations considering also vacuum and mechanical construction.
The final design consists of a ferrite ring (inner diameter = 150\,mm, radial 
width = 15\,mm, thickness = 5\,mm) integrated into the 
flange, as far as possible from the beam %(Figure~\ref{fig:cyl_ferrite}).
%This design is feasible and can be easily integrated in the existing design.

%
%\begin{figure}[h!]
%\begin{center}
%\includegraphics[height=6cm]{figs/detector/Ferrite5x15.jpg}
%%\vspace*{5cm}
%\caption{Detail of the geometrical model used in the impedance simulations. It shows the
%new ferrite ring to be integrated in the flanges of the cylindrical pots and of the
%improved pots with shields. 
%}
%\label{fig:cyl_ferrite}
%\end{center}
%\end{figure}
%
%Figure~\ref{fig:Zlong} shows the real and imaginary parts of the longitudinal impedances
%of the three RP designs with ferrites. 
In all cases, the 470\,MHz resonance is damped and
smeared beyond recognition. At low frequencies, the cylindrical and shielded RPs have 
a smaller $\Re [Z_{\rm long}]$ than the standard RP. This is also reflected by the 
reduced heating for the new designs (Figure~\ref{fig:Ploss_vs_d}).
%
%\begin{figure}[h!]
%\begin{center}
%\includegraphics[width=0.495\textwidth]{figs/detector/ZBox.jpg}
%\includegraphics[width=0.495\textwidth]{figs/detector/ZCyl.jpg}\\
%\includegraphics[width=0.495\textwidth]{figs/detector/ZShield.jpg}
%%\vspace*{5cm}
%\caption{Simulated longitudinal impedance for the standard box-shaped RP (top left), 
%the cylindrical RP (top right) and the shielded RP (bottom). 
%Both real and imaginary part are shown.
%}
%\label{fig:Zlong}
%\end{center}
%\end{figure}
%
%
\begin{figure}[h!]
\begin{center}
\includegraphics[width=0.495\textwidth]{figs/detector/PlossCyl.jpg}
\includegraphics[width=0.495\textwidth]{figs/detector/PlossShield.jpg}
%%\vspace*{5cm}
\caption{Power lost by the beam passing through the RP, for the three RP designs ($I=0.6$\,A).
}
\label{fig:Ploss_vs_d}
\end{center}
\end{figure}
%
Figure~\ref{fig:Zlong_vs_d} shows the effective longitudinal impedance as a function of 
the RP distance from the beam. Also here, the new designs have led to a significant 
reduction.
%
\begin{figure}[h!]
\begin{center}
\includegraphics[width=0.495\textwidth]{figs/detector/ZlongCyl2.jpg}
\includegraphics[width=0.495\textwidth]{figs/detector/ZlongShield2.jpg}
%%\vspace*{5cm}
\caption{Effective longitudinal impedance as a function of 
the RP distance from the beam, for the three RP designs.
}
\label{fig:Zlong_vs_d}
\end{center}
\end{figure}


These results are numerically summarised in Table~\ref{table:impedances}.
%
\begin{table}[!ht]
\footnotesize
\centering
\renewcommand{\arraystretch}{1.5}
\begin{tabular}{|p{0.14\textwidth}|p{0.13\textwidth}|p{0.09\textwidth}|p{0.11\textwidth}|p{0.09\textwidth}|p{0.11\textwidth}|p{0.09\textwidth}|}
\cline{1-7}
		&	Distance from the\newline beam [mm]	&	$\frac{\Im Z^{0}_{\rm long}}{n}$ [m$\Omega$] &	fraction of $(\frac{\Im Z_{\rm long}}{n})^{\rm eff}_{\rm LHC}$ (90\,m$\Omega$)	&	$\overline{\Im Z_{\rm trans}^{\rm driving}}$ [M$\Omega$/m]
		& fraction of $\Im (Z_{\rm x})^{\rm eff}_{\rm LHC}$ (25\,M$\Omega$/m)		&	Heating [W] I=0.6~A\\
	\cline{1-7}
	\multirow{3}{1cm}{\centering \mbox{Box RP}}			&	1		&	1.7					&	$< 1.9$\,\%				&	0.15							&	$< 0.6$\,\%				&	62 \\
								&	5					&	1.3					&	$< 1.4$\,\%				&								&							&	52 \\
								&	40 (garage)				&	 0.41					&	$< 0.45$\,\%	 			&								&							&	10 \\
	\cline{1-7}
	\multirow{3}{1cm}{\centering \mbox{Cylindrical RP}}		&	1			&	1.1		 			&	$< 1.2$\,\%				&	0.11							&	$< 0.5$\,\%				&	13 \\
								&	5					&	0.73					&	$< 0.81$\,\%				&								&							&	11 \\
								&	40 (garage)				&	0.18					&	$< 0.20$\,\%				&								&							&	4 \\
	\hline
	\multirow{2}{1.5cm}{Shielded RP}		&	1					&	1.2					&	$< 1.3$\,\%				&	0.2							&	$< 0.8$\,\%				&	10 \\
								&	40 (garage)				&	0.30					&	$< 0.33$\,\%				&								&							&	2 \\
	\cline{1-7}
	\end{tabular}
\caption{Main results of the simulation of the present box RP (Box RP), the cylindrical RP (Cylindrical RP), and the Box RP with Shield. Longitudinal and transverse impedances are compared with the total values estimated for the present LHC effective impedances.}
\label{table:impedances}
\end{table}


\subsubsection{The RF Test in the Lab}
The new cylindrical RP and the RF shield in combination with ferrites were developed to reduce the 
RF interaction with the LHC beam. 
Prior the serial production of components a new RP cross with flanges and bellow
was manufactured. The prototype of the cylindrical RP and the RF shield in 
combination with the box-shaped RP have been integrated in this new  RP cross for RF measurements. 
Starting from February 2014 measurements were performed by TOTEM and the LHC impedance group in the TIF lab of CERN. In detailed measurements with and 
without the new ferrites and at different insertion positions of the RP, the RF characteristics of this new geometry could be determined and good agreement 
with the predictions, based on simulations could be found~\cite{note_rprf}.


\subsubsection{Impact of Ferrite outgassing on LHC Vacuum}
The vacuum degradations observed in 2012 after very close horizontal RP 
insertions to high-intensity beams triggered the following consolidation
activities for improving the vacuum compatibility of the RP system:
\begin{itemize}
\item Ferrite material improvements:\\
The 4S60 ferrites used in the RP system before LS1 are now (but not in 2006) 
known to show high outgassing rates unless they are baked out at 
1000$^{\circ}$C~\cite{gregory_test1}.
In the TOTEM RPs these ferrites were installed as received from the 
manufacturer and then baked out \textit{in situ} at about 200$^{\circ}$C like all
other beam-pipe components, which turned out not to be sufficient.
Since the 4S60 ferrites have in addition a low Curie temperature of only  
100$^{\circ}$C, alternative ferrite materials are being investigated instead of 
only baking out the 4S60 material at 1000$^{\circ}$C.
The material used for the TOTEM RPs is TT2-111R from 
TransTech with a Curie temperature of $375^{\circ}$C and an acceptable 
outgassing after bake-out at 1000$^{\circ}$C~\cite{gregory_test2}.
An alternative material 
for possible future use is
4E2 (Ferroxcube) with a Curie temperature
of about $400^{\circ}$C; its outgassing behaviour remains to be tested.
\item The new geometrical ferrite configuration reduces the ferrite surfaces exposed
to the vacuum by an order of magnitude from 220\,cm$^{2}$ per standard RP to 23\,cm$^{2}$
per cylindrical RP.
\item All components exposed to the primary beam vacuum have been proposed
by the vacuum group to be coated with NEG, as far as technically possible.
\end{itemize}

\subsubsection{Generation of Particle Showers}
\label{sec:showerMC}
To assess the generation of particle showers by RPs interacting with the 
intense debris halo (see 2012 experience discussed in 
Section~\ref{sec:beamenvironment2012}), Geant4 simulations implementing 
detailed models of the rectangular and the new cylindrical RPs 
have been carried out~\cite{frici_note}. 

The first goal of the study was to identify the contributions from the 
different structural elements of a RP to the shower creation.

As expected, the number of secondary particles is mostly determined by the 
amount of material traversed. The key observations are:
\begin{itemize}
\item 
In both RP designs, the bottom foil produces by far the highest number 
of secondary particles, followed by the thick body walls with 2 to 3.5 orders 
of magnitude lower rates. The orthogonally traversed thin front and back windows
produce the lowest numbers of secondaries.
\item 
The bottom foil of the cylindrical pots produces more than 10 times more 
secondaries than the much shorter foil of the standard pots. In the other 
elements the shower production is similar in the two designs.
\item
The showers from the bottom foil of the cylindrical pot are 3 times 
wider than the ones
from the standard pots: 99\% contained in 0.6\,rad$\,=34^{\circ}$  rather than in 0.2\,rad$\,=11^{\circ}$.
\item
The two projections, horizontal and vertical, are almost identical.
\end{itemize}


The simulated secondary 
particle distribution in a scoring plane 6\,m
downstream of a standard horizontal RP inserted to 2\,mm from the beam centre
shows that
at the entrance point of TCL6,
25\,\% of the secondary particles, carrying 90\,\% of the energy, are contained within the beam-pipe radius and thus 
intercepted by TCL6. How much of this flow leaks through the TCL6 aperture and
thus hits Q6 will be the subject of the FLUKA study discussed in 
Section~\ref{sec:collimation}.



%----------------------------------------------------------------------------

\subsubsection{Interplay between Roman Pots and Collimators}
\label{sec:collimation}
The modified RP system with relocated and additional units will be 
embedded in an upgraded collimation system. This section discusses the 
performance of the new combined layout in terms of physics acceptance and 
machine protection.

\paragraph*{The New Collimators TCL4 and TCL6}

LHC operation at highest luminosities may require additional protection of 
the quadrupoles Q5 and Q6 against collision debris from IP5~\cite{stefano}.

To protect Q5, new collimators, TCL4, have been installed on the outgoing beams
in the old location of the RP147 station, and the already existing collimators
TCL5 may be partially closed. Since both TCL4 and TCL5 are located upstream of
the RP stations and can intercept diffractive protons if too tightly 
closed, the aperture settings of these collimators will be the
result of an optimisation study maximising the physics acceptance as far as 
compatible with the necessary magnet protection.

Downstream of the last RP unit, 220-F, another collimator, TCL6, has been
installed~\cite{ecrcollim} on the outgoing beam to protect the quadrupole Q6 against 
debris from IP5, thus taking over a part of the original role of TCL5 
which cannot be too tightly closed without intercepting all the signal protons 
to be measured by the RP system. Another beneficial effect of this new 
collimator is its capability to absorb showers created by the insertions of 
the horizontal RPs close to the beam. RP operations at low $\beta^{*}$
and high luminosities in 2012 have demonstrated that without any absorber 
behind the RP stations, insertions were limited to distances greater than 
30\,$\sigma$, because the showers caused by the pots' interaction with the 
debris halo brought the dose rates measured by the Beam Loss Monitors above 
the beam dump thresholds. The improvement by the addition of TCL6 will be 
the subject of a FLUKA study.


\paragraph*{Optimisation of Roman Pot and Collimator Settings}

This section discusses the strategy for defining an optimal combined set of jaw 
positions for the RPs and the collimators TCL4, TCL5 and TCL6. Given that 
the TCLs are only required at highest luminosities, only the low-$\beta^{*}$
running scenarios are relevant for these considerations.
The TCL collimators are designed to protect the quadrupoles Q5 and Q6 against
debris from collisions at IP5. Their jaws approach the beam 
horizontally and potentially intercept diffractively scattered protons, thus
interfering with the physics measurements in the RPs.
Therefore, the aim of the optimisation is to find 
\begin{enumerate}
\item jaw positions for TCL4 and TCL5 that leave the aperture as widely open as 
allowed by the protection needs of Q5, i.e. the dose rate received by Q5 has
to stay well below the magnet quench threshold;
\item RP positions as close to the beam as allowed by the protection
capacity of TCL6 to prevent Q6 from quenching.
\end{enumerate}
The upper limit $\xi_{\rm max}$ for accepted momentum losses of diffractive 
protons is given by minimum value of the ratio $d_{x}/D_{x}$ between horizontal 
aperture and dispersion along the path from the interaction point to the RP.
Table~\ref{tab:apertures} gives the values of $10\,\sigma_{x}$ beam width and
the dispersion $D_{x}$ in all TCL collimators and in some RP locations for the 
$\beta^{*} = 0.55\,$m optics at $\sqrt{s}=14\,$TeV.

\begin{table}[h!]
\begin{tabular}{|l|c|c|c|c|}
\hline
Beam Element & Position $s$ [m] from IP5 & $10\,\sigma_{x}(s)$ [mm] & $D_{x}(s)$ [mm] & $|\xi(10\,\sigma)|$\\
\hline
TCL4         & 149                       & 5.2       & -66   & 0.079 \\
TCL5         & 185                       & 2.8       & -83   & 0.034 \\
RP 210-N     & 202                       & 2.2       & -90   & 0.024 \\
RP 220-F     & 220                       & 0.90      & -80   & 0.011 \\
TCL6         & 221                       & 0.89      & -80   & 0.011 \\
\hline
\end{tabular}
\caption{Horizontal beam envelope ($10\,\sigma$) and dispersion at the TCL 
collimators and at the first and last RP unit. The last column gives the 
$\xi$-value at $10\,\sigma$ from the beam centre (for $t=0$).
}
\label{tab:apertures}
\end{table}
%
The most stringent impact on diffractive proton acceptance is made by TCL5
which at its nominal jaw position of $10\,\sigma$ from the beam centre would 
intercept all protons with $\xi>0.034$ while for the physics programme a 
cut-off greater than 0.1 would be desirable. 
Therefore collimation group developed an alternative
scheme for fills with RP operation where TCL5 would be fully open and both 
TCL4 and TCL6 closed to $10\,\sigma$. However, in that scheme TCL4 would 
be the bottleneck producing a cut at 0.079. A new study presently carried out
by the FLUKA team investigates the possibility to open TCL4 to $15\,\sigma$
and complement its protection by closing TCL5 to $35\,\sigma$. In this way, 
both collimators would lead to the same upper $\xi$ cut-off at 0.11.

Once the optimal settings for TCL4 and TCL5 will be fixed, another FLUKA study
will focus on the impact of RP insertions on Q6 and its mitigation by closing
TCL6 to $10\,\sigma$. It is expected that a horizontal RP approach to 
a minimum distance between 11 and $14\,\sigma$ should be possible, corresponding
to minimum accepted $\xi$-values between 0.012 and 0.016.


\subsection{Requirements on the Timing Detectors and Strategy}
\label{sec:timing_cherenkov}
 
The need for precise timing detectors measuring the time difference of the
protons in the two arms of the spectrometer is justified 
%in Chapter \ref{sec:??????} 
as an effective way to reduce the pileup background. 
A baseline time resolution of $\sigma(t)=10$\,ps, corresponding to
a vertex resolution $\sigma(z_{pp})=2.1$\,mm, is set as an ambitious target of the CT-PPS project.
%A backup scenario where the time resolution is limited to a conservative value
%of 30\,ps is also evaluated and justified in the physics performance studies
%presented in Chapter~\ref{sec:?????????}.

The required detector area is small ($\leq4\rm cm^2$). In addition to a good time resolution, 
the use of a detector with a small dead region is a key requirement.  On the
side adjacent to the beam, the dead region should be at the level of $ \sim 200\,\mu$m or below, matching that of the tracking detectors. The distance between
the active area and the vacuum includes in addition the bottom of the RP
($0.3^{+0.02}_{-0.10}$\,mm). The scattered protons are deflected out of the 
beam by the LHC magnets, but at the $z$ position 
of the detectors they are displaced by only a few mm, so any inactive area (on the inner edge) 
causes a loss in acceptance at low masses.

The detectors should be radiation hard. Close to the beam where the detectors
are located, we expect a proton flux of about $5 \times 10^{15}\rm\,cm^{-2}$ per
100\,fb$^{-1}$. The expected thermal neutron flux extrapolated from TOTEM measurements is about
$10^{12}\rm\,cm^{-2}$ per 100\,fb$^{-1}$. In the case of Cherenkov detectors the
photodetectors will be farther from the beam, where radiation field is reduced to the neutron component. 
Replacing the photodetectors or solid-state timing detectors approximately once a year is feasible, 
as they are accessible and relatively inexpensive.

As there is often more than one proton in the acceptance from the same bunch crossing, 
a fine segmentation is also required. The detectors should have the capability
of measuring the times of two or more particles from the same bunch crossing, and of being read out every 25\,ns, 
with no significant remnant signals from earlier crossings. This implies segmentation. 

A detector based on Cherenkov technology is developed for precise timing as the
baseline proposal. 

%Similar technology was studied earlier in the context of the 
%FP420 project R\&D project~\cite{fp420}. 
%These included detectors based on quartz (or sapphire) radiators as well as gas
%Cherenkov detectors. Several prototypes have been built and evaluated in test beams.
%Recently there has been growing interest in timing measurements, which has led
%to several on-going R\&D efforts on the use of solid state detectors for timing, 
%notably in the frame of the LHC Phase 2 Upgrade programme. Several CT-PPS groups are 
%participating to these efforts and are willing to explore the option of using such detectors in PPS.

Presently, the state-of-the-art of time resolution with minimum ionizing
particles in a single detector layer is the following:
1) gas Cherenkov $\sim$\,15\,ps~\cite{gastofnim}; quartz Cherenkov $\sim$\,30\,ps
\cite{clermont}; diamond sensors $\sim$\,100\,ps \cite{diamond,diamond2};
silicon sensors $\sim$\,100\,ps \cite{silicontiming}. Complete systems with several detector
layers allow for improved performance.

While Cherenkov based detectors have intrinsically better time resolution and are more mature timing 
technologies, they have some important drawbacks. In the existing prototype implementations, the quartz 
detector is segmented in elements of $3\times3$ mm$^2$, which implies a large
rate of double hits in the same bar per bunch crossing, approaching 50\% in the
sensors close to the beam. We assume that two hits in the same channel cannot be resolved. 
%This source of inefficiency is taken into account in the physics performance simulations in Chapter\ref{sec:??????????}.  
Finer granularity near the beam, where it is most
needed, may be possible but needs further development.

The amount of material introduced by the quartz detector itself is not negligible. In the foreseen 
configuration, the probability that a proton has a nuclear interaction in one
detector is between 7.2\% and 14.6\% (depending on the proton position in the
detector). As the timing detector is located downstream of the pixel detectors  these 
interactions do not affect the track measurement, however they may smear or fully corrupt 
the time measurement introducing another source of inefficiency.

%The gas Cherenkov detector is not affected by this issue, but on the other hand its granularity 
%is only indirect, in the sense that a multi anode Micro Channel Plate
%photomultiplier (MCP-PMT) could possibly allow to disentangle Cherenkov photons
%from different protons. Indeed the reconstruction of the time of two or more protons in 
%the detector is affected by the uncertainty in associating MCP-PMT channel
%information to individual protons.
%This question is investigated with GEANT simulation (\cite{ctpps-tdr}, Section~5.3).
%The MCP-PMT devices have also a limited life time in terms of integrated charge,
%which requires using the device at reduced gain, preventing the optimal time
%resolution.

Solid state timing detectors have the important advantage of being very thin and allowing for fine 
granularity. Typically solid state detectors are a few hundred microns thick
making it possible to stack ten or more detectors, which to a first
approximation improves the time resolution by the square root of the number of layers. A 
resolution of 30\,ps per detector, possibly achieved as a result 
of the current R\&D effort, would allow for a timing system with the baseline 10\,ps resolution. On the other hand the possibility of defining small size pixels permits 
reducing the rate per channel, 
which improves 
the time measurement and reduces significantly the inefficiency due to double hits. Of course the 
detectors should be able to sustain the high radiation doses involved in this
application, which requires still considerable development.  

Taking into account the previous considerations, we have chosen as
the baseline timing detector the L-bar Quartic (Quartz Timing
Cherenkov) design with $5\times4 = 20$ independent
channels of $3\times3\rm\,mm^2$ area. The SiPM photodetectors are relatively far from the beam, in 
a region where the neutron flux is $\sim 10^{12}$\,neq/cm$^2$ per 100\,fb$^{-1}$.
SiPM devices that tolerate this radiation level are available, as found in
the framework of the HCAL Upgrade project, however a
increase of the leakage current is observed~\cite{hcal_upgrade}. The SiPMs will
probably require replacement after 100\,fb$^{-1}$, which is feasible given the small number of
devices involved. We will also consider the possibility of using GaInP
photosensors, under development for the upgrade of the CMS endcap calorimeter,
given its potentially better tolerance to radiation. Two Quartic detectors
fit inside a cylindrical Roman Pot, providing a combined resolution of the order of 20\,ps. 
The Quartic baseline is presented in Section~\ref{sec:quartic}.

The relatively high fraction of nuclear interactions in the quartz bars prevents
the use of more than two Quartic detectors per spectrometer arm. In order to reduce the amount of the dense
material, we explore the possibility of complementing the Quartic measurement
by using a short ($\sim 10$\,cm) Gas Cherenkov Time-of-Flight detector (GasToF)
inside a second, upstream, cylindrical RP.
The GasToF detector with a multi-anode MCP-PMT may be able to time individual
photoelectrons to achieve multi-proton capability. Combined with the Quartic measurements, this additional 
detector could allow 
to approach the 10\,ps time resolution. While GasToF prototypes have been built
and validated, there are not yet test beam results confirming the multi-hit performance predicted 
from simulation. The possible use of GasToF 
in the experiment is therefore dependent on successful test beam results with final prototypes. The 
GasToF option is described in~\cite{ctpps-tdr} (Section~5.3).

Both the Quartic and GasToF detectors have a relatively small number of channels
and produce electrical pulses with similar characteristics. Therefore the proposed readout system, based on two well 
known integrated circuits (the amplifier-discriminator NINO and the High
Performance time-to-digital converter HPTDC), can be used by
both detectors. This solution offers a potential for possible future upgrades
as new improved versions of the HPTDC and of the NINO chips are already in the
pipeline.
A reference clock system, complementary to the CMS timing system, provides time synchronization 
with less than 1\,ps jitter between the detectors in opposite arms.  
%Sections~\ref{sec:timing_electronics} and \ref{sec:?????????} describe the
%Cherenkov readout system and the reference timing system, respectively.

In parallel we intend to pursue the R\&D on solid state options for timing, in
particular diamond sensors and silicon sensors with avalanche gain. There are still many challenges to overcome 
before any of these options become a viable timing detector for CT-PPS. This includes the improvement 
of the intrinsic detector resolution, the demonstration of resistance to radiation, and the development 
of suitable low noise and fast electronics. Prototypes will be built and evaluated in test beams. 
The small area, and therefore cost, of the timing detectors allows to foresee the replacement of the 
CT-PPS timing baseline when a better solution is available. 
The solid state options and respective R\&D plans are described in~\cite{ctpps-tdr} (Sections~5.5 and~5.6).



\subsubsection{The Cherenkov Quartic Detector as Baseline for Timing}
\label{sec:quartic}
%  
Cherenkov light is prompt and therefore ideal for fast timing, although the amount of light is small
compared to that in scintillator. Radiators need to be transparent, i.e. with a long absorption length
$L_{abs}(\lambda)$, where $\lambda$ is the optical wavelength, preferably into the
ultraviolet, $\lambda \approx$ 200\,nm, where most photons are generated.  The
number of Cherenkov photons radiated is proportional to $1-1/n^2(\lambda)$; more completely
(for charge $Q = 1$, and $\beta = 1$):
\begin{equation}
\frac{d^2N}{dxd\lambda}=\frac{2\pi\alpha}{\lambda^2}\left(1-\frac{1}{n^2(\lambda)}\right) \: ,
\end{equation}
where $\alpha$ is the fine structure constant.

The approximate rule for the number of photoelectrons in a typical detector is:
   \[N_{pe} \sim 90 \: \mathrm{cm}^{-1} \cdot \mathrm{L(cm)\: sin}^2 \theta_{ch} \sim 50\; \mathrm{cm}^{-1},\]
    which gives about 200 photoelectrons for a quartz detector of length 40 mm, to be scaled by a factor for the acceptance of the photons. 
 

The light is emitted along the particle's path in a cone
with half angle (Cherenkov radiation angle) $\theta_{ch}$ given by cos$(\theta_{ch}) = 1/n(\lambda)$.
We have developed fast detectors with both gas and solid radiators.
%The gas Cherenkov detector, or GasToF, is described in~\cite{ctpps-tdr} (Section~5.3).
%The Cherenkov light is much smaller than in a solid radiator but is very collimated. It is detected with a 
%MCP-PMT,
%and by timing individual photoelectrons one can measure the time of more than one proton 
%from the same bunch crossing. 

 Among solid radiators, fused silica, SiO$_2$, or quartz
(ultraviolet grade, UVT) is commonly used, and it is chosen as our baseline material. As $n(\lambda) \sim 1.48$, there 
is much more light per cm than in a
gas, but since $\theta_{ch} \sim 48^\circ$, the light does not arrive as
promptly, and fine segmentation, in our case with quartz bars, is limited. 
%The refractive index of quartz varies from 1.455 at $\lambda = 700$\,nm to 1.475 at $\lambda = 350$\,nm. The corresponding Cherenkov angles 
%are $46.6^\circ$ and $47.3^\circ$. Over this wavelength range the optical absorption length of quartz is $> 110$\,cm. 
%The density of quartz is 2.20\,g/cm$^{3}$, the radiation length is 12.3\,cm and the interaction length $\lambda_I = 44.5$\,cm. 
   
 
 
\subsubsection{Quartic Design for Roman Pots, with L-Bar Geometry}
%

We have developed detectors \cite{Albrow-ARX-2012} with quartz bars of 
$3 \times 3\rm\,mm^2$ cross section in the form of an `L', called L-bar Quartic
(QUARtz TIming Cherenkov), the light being detected with SiPMs. 

This configuration allows segmentation in both $x$ and $y$. 
  The photodetectors are located at $\sim 8$\,cm from the beam in the horizontal plane and can be 
  partially shielded to reduce their radiation dose.%
{(\bf need to be rephrased to avoid repetitions)}

In the Quartic design 
there is an array of $3 \times3\rm\,mm^2$ ``radiator bars'', R, parallel to the beam. 
The Cherenkov angle is the complement of the critical angle for Total
Internal Reflection (TIR) on the bar sides, and as the proton paths are almost exactly parallel to the bars all the Cherenkov
light is internally reflected to the back end of the radiator, as shown schematically in Figure~\ref{lbarsketch}. 
Most (about 2/3) of the light is transmitted to the SiPM along 
the light-guide (LG) bar, also with total internal reflection. The remaining $\sim 1/3$ is
reflected back to the entrance of the radiator bar, where there will be a black absorbing surface. 
The LG bars end in a (vertical in the horizontal RP) plane, 73\,mm from the beam pipe wall. 
This distance is a compromise between being away from the
beam for radiation issues, and keeping the LG bars short to minimise the absorption, 
number of reflections, and optical dispersion.
The spread of the travel time of the photoelectrons is mainly caused by the length of the 
radiator bar. The component of the speed of the light along
the radiator bar is $dz/dt = c/n^2 \sim 0.140$\,mm/ps. 

\begin{figure*}[t]
\centering
\includegraphics[width=70mm]{figs/detector/lbardiag2.jpg}
%\vspace*{5cm}
\caption{Cherenkov light rays in the radiator and light guide bar, for $n$ = 1.48, in the plane of the `L'
 ($\phi_{ch} = 90^\circ$).}
 \label{lbarsketch}
\end{figure*}

%Sapphire, Al$_2$O$_3$, has a higher refractive index, $n \sim 1.78$ and hence about 27\% more light per cm, however it is denser and has a 
%shorter nuclear interaction length ($\lambda_I = 24.8$\,cm cf. 44.5\,cm). To minimize interaction issues we choose quartz.
%Our baseline is to have two Quartic modules per arm, in one RP. 
% The second RP foreseen for timing detectors can be used for housing a GasToF or solid-state timing
%detectors. In both cases, the alternative timing detectors will be installed upstream of the Quartics, 
%to provide complementary time measurements. 
Detailed studies of the Quartic and other timing detectors can be found in  Refs.\cite{clermont,Albrow-ARX-2012,mazzillo,ronzhin,vavra}. 
 
% Figure~\ref{twobarbox} shows the design of a test module, with two 30\,mm and
%two 40\,mm bars in line, used in beam tests at Fermilab~\cite{Albrow-ARX-2012}. The beam comes from the right, 
%and the two SiPM boards, each with two SiPMs,
%are at the top in the figure.
%The radiator bars were separated by 100\,$\mu$m wires and held in place by plates with narrow ridges 
%such that they only minimally touch the bars.
%The distance between the LG bars was dictated by the borders of the SiPMs. It results in different 
%R-bar and LG-bar lengths. SiPMs with thinner borders
%(``buttless'') are becoming available and could reduce this spread in lengths. A feature of the 
%design is that protons through the shorter R-bars, farther from the
%beam, also traverse the LG-bar of the longer bars. Half of the Cherenkov light emitted in LG bars 
%is totally internally reflected to the SiPM; 
%In the case of a single particle in the
%detector from one bunch crossing the extra signal can be used, but in the case of two or more protons it has the 
%undesirable effect of reducing the efficiency.  
%The results of these beam tests are described in Section~\ref{sec:beamtest}.

%\begin{figure*}
%\centering
%\includegraphics[width=80mm]{figs/detector/boxdesign.jpg}
%%\vspace*{5cm}
%\caption{Design of an L-bar box with two modules, each with two L-bars, as used in the tests. The beam comes from the right, and the 
%SiPMs are at the top.}
%\label{twobarbox}
%\end{figure*}

%We then made a module with an $4\times 5$ array of quartz bars with an
%``edgeless design'', appropriate for a MBP. This was valuable
%in enabling us to solve many practical issues arising with a compact, edgeless array. Beam tests (not expected to show different resolution from the earlier two-bar module) showed light leakage between the bars, resulting in reduced efficiency, and
%leading us to increase the inter-bar spacing from 100\,$\mu$m to 200\,$\mu$m for the actual device.
%Since the first stage of the CT-PPS project is to use horizontal RPs, we modified the Quartic design.
%The RPs assigned for the timing detectors have longitudinal
%  space 140\,mm and the Quartic detector is designed such that two can fit in one RP. It should be noted that while multiple scattering of the 
%  protons is not an issue, as the tracking stations are upstream, the effect of inelastic interactions can be important. If an inelastic interaction occurs 
%  the signal in that and any following detectors is likely to
%  be large and spread out in time, as well as not being confined to one bar. 
     

   
The CT-PPS Quartic ``module'' 
is a light tight box with a very thin ($\sim 100\,\mu$m) side wall on the beam side, and blackened interior. 
This side wall may be removed on insertion in the pot as the interior will be dark; it is to protect the inside prior 
to insertion and to optically close the
box for beam tests. One module consists of ($4 \times 5 = 20$) independent $3 \times 3\rm\,mm^2$
bar elements. This allows a time measurement of two or more protons from the same bunch crossing (which has a 
time spread $\sigma_t \sim 150$\,ps) if they are in different elements. The active area is 12.6\,mm
(vertically, $y$) $\times$ 15.8\,mm (horizontally, $x$).  
This includes 200\,$\mu$m spacers (a wire grid) 
to separate the bars, allowing total internal reflection, and avoiding light leakage.
The dimensions of the bars are given in Figure~\ref{fig:barl}.
    The ends of the light guide bars arrive at an array of SiPMs, coupled with a thin 
    silicon ``cookie'' for good optical coupling. 
    We use SiPMs Hamamatsu MPPC Type S12572-050 mounted in a flat plate
    holder (3D-printed plastic). The SiPMs fit in
   rectangular holes in the plate
   and as they are not fixed to the read-out board they can be very simply
   replaced. 
    The SiPMs are connected to the read-out board through
   an anisotropic conducting sheet (embedded very short wires give an electrical connection through 
   the sheet but not in the plane).  
  
\begin{figure}
\centering
\includegraphics[width=120mm]{figs/detector/compactinpot.pdf}
%\vspace*{5cm}
\caption{Schematic layout of quartz bars looking in the direction of the protons. 
Numbers on the $3 \times 3\rm\,mm^2$ radiator bars are their lengths in mm, and
coordinates (mm) are the centers of the bars. The light guide bar lengths are chosen to all end in a common 
plane 81.7\,mm from the edge closest to the beam.}
  \label{fig:barl}
\end{figure}
  
%Figure~\ref{linediag} shows isometric views of a module. The front view shows the 4 (in $y$) $\times$ 5 (in $x$) 
%bar array, and the top view shows the position of the
%LG bars (in precise round holes in a plate). 
%The side view shows a removeable inspection plate, not needed inside the pot. Figure~\ref{sipmplan} shows the 
%design of the SiPM read-out board. 

%\begin{figure}
%\centering
%\includegraphics[width=120mm]{figs/detector/linediag.png}
%\vspace*{5cm}
%\caption{Design of the Quartic module for the Roman pot. The bottom right figure is the front (proton's) view, with the
%beam to the right. The top left shows the light guide bars at the SiPM plate.}
%  \label{linediag}
%\end{figure}


%\begin{figure}
%\centering
%\includegraphics[width=100mm]{figs/detector/sipmbd.png}
%\vspace*{5cm}
%\caption{Design of SiPM readout board (s.Los). Three of the multi-way connectors J25 - J28 are for the high voltage and one for monitoring leakage currents and temperature.}
%\label{sipmplan}
%\end{figure}

 
%Figure~\ref{box1} shows a 3D view of the module. 
%It is 68\,mm long, so
%  that so that two modules can be installed in one RP (140\,mm in $z$). The
%  U-shaped holder near the front of the bar-array, holds them in place with
%  screws applying a little pressure, but only touching along a (3D-printed) ``knife edge''. The bars are separated from each other (and from the bottom of the pot) by a 200\,$\mu$m wire grid.
%  A similar frame will position the LG bars, which also pass though a 3D-printed positioning plate.
%  The bottom plate (not shown in this figure) is not structural and can be removed. The complete block of bars is inserted as a unit (with temporary clamps) from that side. 

 The bars pass through circular holes for locating the
bars against the SiPMs, with better than 25\,$\mu$m accuracy. These holes are countersunk, as the 20 bars all have to be inserted together.
The U-clamp is then tightened and the temporary clamp removed. The complete bar assembly is then slid into the box on precision grooves; the front
window is placed in position later, after position and optical checks are done. 
%Figures~\ref{twoinpot2} and~\ref{twoinpot} 
Figure~\ref{twoinpot} shows the assembly of two modules in one RP. 
We have the option of displacing one module in $(x,y)$ with respect to the other by 250\,$\mu$m (e.g.) to avoid any dead regions between
the bars. Alignment of the radiator bars parallel to the protons (at the level of $\lesssim 10$\,mrad) will be needed to maximise light collection and avoid light leakage into neighbouring bars.

\subsubsection{Integration with Roman Pots}
%

{(\bf check for repetitions)}

The longitudinal space in the RPs is approximately 140\,mm. The L-bar geometry 
allows installation of Quartic two modules in one RP(Figure~\ref{twoinpot}) %(Figures~\ref{twoinpot2} and~\ref{twoinpot}). 
The two modules in a pot will be fitted together precisely using dowel pins. 

%Figures~\ref{linediag} and~\ref{box1} 
Figure~\ref{twoinpot} 
shows the design of the module for insertion into the horizontal RP. 
A slightly modified version (Figure~\ref{pev}) reduces the material close to the beam.
The protons enter through a thin
window (nominally 100\,$\mu$m aluminium, but it has no mechanical purpose, it is for absorption of reflected light and light exclusion). 
The array of radiator bars
is clamped on the three sides away from the beam with a plastic U-clamp, touching each bar only along a fine line. 
For assembly of the bar array a 4-sided clamp is placed temporarily 
around the front of the array. 
The SiPM plate and read-out board are precisely positioned by dowels with respect 
to the L-bar positioning plate.

    
\begin{figure*}[hp]
\centering
\includegraphics[width=0.49\textwidth]{figs/detector/box1_rot.png}
%%\vspace*{5cm}
%\caption{Design (B. Ellison, FNAL) of module for insertion in Roman Pot (two in one pot).}
%\label{box1}
%\end{figure*}
%\begin{figure*}[ht]
%\centering
%\includegraphics[width=78mm]{figs/detector/twoinpot3.png}
%%\vspace*{5cm}
%\caption{Assembly of two Quartic modules in Roman Pot.}
%  \label{twoinpot2}
%\end{figure*}
%\begin{figure*}[ht]
%\centering
\includegraphics[width=0.49\textwidth]{figs/detector/twoinpot.png}
%%\vspace*{5cm}
\caption{Left:Design (B. Ellison, FNAL) of module for insertion in Roman Pot (two in one pot). Right: Assembly of two Quartic modules in Roman Pot. The beam comes from the left.}
  \label{twoinpot}
\end{figure*}

\begin{figure*}[ht]
\centering
\includegraphics[width=80mm]{figs/detector/closefit.png}
%%\vspace*{5cm}
\caption{``Particle eye view'' of bar array in pot. This is a modified design (D. Druzhkin) reducing the material close to the beam.}
  \label{pev}
\end{figure*}



\subsubsection{Photodetectors: Silicon Photomultipliers}
%
     Silicon photomultipliers, SiPMs, are solid state photon counters comprised of a large number of avalanche 
     photodiodes (APDs) or ``pixels" of order 20\,$\mu$m
     dimensions, 
     with a high gain (up to $10^6$) in Geiger mode, with an applied voltage just above the breakdown 
     voltage (about 30\,V to 70\,V depending on the type).
     Each discharged pixel has a recovery time of $\sim 50$\,ns, but with e.g.
     100 photoelectrons per event and thousands of pixels per mm$^2$ this is acceptable with 25\,ns bunch-crossing time. For the SiPMs, the single photon detector efficiency is the product of the quantum efficiency 
     and the fractional area coverage of the APDs. SiPMs are rugged, simple to use and relatively
     cheap per unit, but at present are only available
     commercially with effective active areas from $1\times1\rm\,mm^2$ to $3.5\times 3.5\rm\,mm^2$. Smaller SiPMs have less capacitance and are
     intrinsically faster. 
 
 The SiPMs, Hamamtsu MPPC type S12572-050,  
 %(Figure~\ref{s12572}), 
 operate at $\sim 72$\,V, 
 just above the breakdown voltage (they operate in Geiger mode, 
discharging one or two pixels per detected photon). These have 3600 pixels of 50\,$\mu$m diameter. 
The single photon detection efficiency and the wavelength-dependence of
the response is shown in Figure~\ref{sipmpde}. Improved efficiency in the UV is being investigated.
Individual HV values can be applied to each SiPM, and their leakage currents monitored
through a high-resistance (6.4\,M$\Omega$) bleed resistor to ground. 
While the gains of SiPMs are very sensitive to temperature, the time resolution is not. Air cooling is 
expected to be sufficient; an alternative is to use the same cooling system as
for the tracking detectors. The temperature of the SiPM boards will be monitored with thermistors. 
The SiPM board receives an individually controllable bias voltage $\sim 72$\,V from a local programmable supply. 
The signals are read out with miniature coaxial cable with SMA connectors.

%\begin{figure}
%\centering
%\includegraphics[width=100mm]{figs/detector/S12572.png}
%\vspace*{5cm}
%\caption{Details of Hamamatsu MPPC (SiPM) S12572-050.}
%\label{s12572}
%\end{figure}

\begin{figure}
\centering
\includegraphics[width=80mm]{figs/detector/SipmPDE.png}
%\vspace*{5cm}
\caption{Photon detection efficiency of Hamamatsu S12572 SiPM. This is the product of the quantum efficiency
and the fill factor (50\,$\mu$m pixels).}
\label{sipmpde}
\end{figure}



\subsubsection{Monitoring, Alignment, and in situ Calibration}
\label{sec:time_align}
The rates in each bar are monitored both online and offline. The
rates are expected to be up-down symmetric about the beam height (as can also be determined from the tracker), 
column-by-column. This gives a measure of the centre of
the beam in $y$, assuming the backgrounds are relatively small. For a given row in $y$ the rates will
fall with $x$ with two components: protons from collisions and beam halo background. The former will be compared 
with predicted $t$-distributions, and it is valuable to
measure the latter. 
When the RPs are inserted at the beginning of stores the rates will be carefully monitored, e.g. 
partially withdrawing in the event
of an abnormal increase.

Initial relative alignment of the Quartic bars and tracker will be achieved by matching the individual bar edges in $x$ 
and $y$ with the track distributions.

A pair of light-emitting diodes will be mounted inside the module in such a way that some light is captured in each bar. 
This will be pulsed when there is no beam as a control
of all the SiPMs and their readout. 

Occupancy of the bars will be monitored in real time, as functions of the instantaneous luminosity 
and background conditions.
Geometrical matching between the
bar array and the trackers will also be measured; the 200\,$\mu$m gaps between the bars can also provide a check. 

A calibration of the absolute time difference between the protons, $\Delta t_{pp}$, can be derived by matching $z_{pp} = z_X$
using real events of the type $p+p \rightarrow p+X+p$, where $X$ is a set of particles measured in the central
   detector. After kinematic matching of $X$ to the protons (four-momentum conservation) the 2D plot of $z_{pp}$ vs $z_X$ will show a ridge which 
   calibrates both $z_{pp} = 0$ as well as checking the time scale. 
   
   While the time difference between the ``left'' and ``right'' protons, $t_L-t_R$, gives $z_{pp}$, the time sum, or $(t_L+t_R)/2$ (minus a constant), 
   would provide another, orthogonal, variable for pileup
   rejection if the actual event time were known much better than the spread in collision times, $\sim$150\,ps. 
 


%\input{ctpps_cher.tex}

\subsubsection{Beam Tests}
\label{sec:beamtest}
%
A prototype Quartic with L-bars was tested in the Fermilab test beam, with 120\,GeV protons, using a mechanical design that does not include
 some features needed for the CT-PPS version. See~\cite{Albrow-ARX-2012} for more details of the test procedures and results. This test module 
 was not edgeless  and had two pairs of bars (separated by only 100\,$\mu$m)
 rather than a $4 \times 5$ block. Two identical modules %(Figure~\ref{twobarbox})
 were placed in line, such that a proton traverses four bars, either 30\,mm or 40\,mm long. The quartz bars were supplied 
by Specialty Glass~\cite{spglass}.
  The photons were detected in a $3 \times 3\rm\,mm^2$ SiPM, the Hamamatsu MPPC S10931-050P with bias 72\,V. 
  The signals were output on SMA connectors. We used a clipping capacitance (9.1\,pF) to shorten the pulse, followed by an ORTEC VT120 $\times$20 preamplifier.
 
% The beam was defined by a $2 \times 2\rm\,mm^2$ trigger counter, and a Photek PMT240 MCP-PMT at the
% back provided a reference time signal with $\sigma_t \sim 8$\,ps. Figure~\ref{drs4} shows the signals 
% recorded in a 5\,GS/s DRS4 waveform digitiser for
% a typical event. The top three traces are the SiPM signals of three 30\,mm
% Cherenkov bars, 20\,mV/div, 2\,ns/div (200\,ps per sample), 
% joined by straight-line
% segments, and the bottom trace (50\,mV/div) is the PMT240 reference signal. 
% Typical pulse heights are about 80\,mV with an 800\,ps risetime. Figure~\ref{phsbar} shows the 
% pulse-height distribution for one bar, 
% consistent with $N_{pe} \sim 50$. The entries in the overflow bin are due to interactions, upstream or in the bar.
% Good timing measurements were obtained by a linear fit to the two points before and 
%  after the 50\% of pulse maximum amplitude, finding
%  the time at which that line crossed the 50\% level, and then applying a time-slewing correction. More complete waveform fits were
%  found to be not significantly better.  
  
%\begin{figure*}[t]
%\centering
%\includegraphics[width=70mm]{figs/detector/scopetrace.jpg}
%%\vspace*{5cm}
%\caption{Waveforms in the DRS-4 of one proton through three L-bars and the PMT240 (bottom trace). The time scale is 2\,ns/div and the vertical scale 20\,mV/div for the top three traces (SiPM's) and 50\,mV/div for the bottom trace (reference PMT240).}
%\label{drs4}
%\end{figure*}
%\begin{figure*}[t]
%\centering
%\includegraphics[width=80mm]{figs/detector/phsbar.png}
%%\vspace*{5cm}
%\caption{Pulse height distribution in a 40\,mm radiator bar. The overflow is due to interactions.}
%\label{phsbar}
%\end{figure*}
 
{(\bf cut a large part of the section as it is not clear and too detailed, check if it is consistent)}

From the spread in signal amplitudes we estimated that the number of
 photoelectrons is $N_{pe} \sim 80-100$. Figure~\ref{deltat} shows, after applying pulse height-slewing 
corrections, the time difference between one bar and the reference time signal, with a time resolution of $\sigma = 35.3$\,ps. After unfolding the electronics and 
reference time resolutions, the time resolution of the 30\,mm bars was $\sim 33$\,ps. Alternatively, 
without using the PMT240 reference time but
comparing the different bar times we found $\sigma_t = 31$\,ps. We
plan to have two modules in-line in one pot, which are expected to give a time resolution of 21\,ps.

After these corrections, the time differences between the four short bars and the reference PMT240 signal had widths, from Gaussian
fits, $\sigma_t = 35 - 40$\,ps, with $\langle \sigma_t \rangle = 37.5$\,ps. 
Figure~\ref{deltat} shows one example, with $\sigma(\Delta t) = 34.9$\,ps, showing no background or inefficiency.
The  single-photon time resolution of the SiPM we used is quoted by Hamamatsu to be $\sim 300$\,ps;
giving an expected time resolution for 100 p.e. of 300\,ps$/\sqrt{100} = 30$\,ps, in reasonable agrement with the observations. 
  

\begin{figure*}[t]
\centering
\includegraphics[width=80mm]{figs/detector/qntdif.png}
%\vspace*{5cm}
\caption{The time difference between one L-bar (30\,mm radiator, 40\,mm light guide, 
  Hamamatsu MPPC type S10362-330050C) and the
  reference time signal (PMT240 in beam). It shows $\sigma = 35.3$\,ps.}
  \label{deltat}
\end{figure*}


\subsubsection{Future Developments}
We have described the baseline Quartic detectors, which could be ready for installation in 2015
when the RPs have been installed and commissioned.  Several potential improvements will be investigated. 
These include finer segmentation, especially near the beam, a more compact SiPM array (``buttless'' type), and the use of a multi-anode MCP-PMT 
in place of SiPMs. The latter have had photocathode lifetime problems limiting their use in such a high-rate environment, but developments 
to mitigate that are encouraging.

Also, faster SiPMs with higher photon detection efficiency and possibly more
sensitivity in the UV may become available, potentially allowing easy replacement.

SiPMs from STMicroelectronics (STM) with new p-on-n structure (rather than N-on-P SiPMs, also from STM) 
show significantly better timing properties~\cite{mazzillo}~\footnote{We thank STMicroelectronics for providing samples.}. 
Tests with a PiLas (Picosecond
Injection Laser) showed the photon
detection efficiency at $\lambda = 405$\,nm, 5\,V above breakdown voltage (28\,V), to be  43\% higher (31.1\% cf. 21.7\%). Also the 
SPTR, is 174\,ps cf. 231\,ps, i.e. smaller by 25\% than for STM n-on-p detectors. 
Together these improvements lead one to expect that the single bar resolution can be improved from the measured 32\,ps to $\sim 20$\,ps.

Unlike the large central CMS detectors, due to the small number of channels,
upgrades to the timing detectors can be considered on a yearly timescale, and we expect to continue the 
necessary R\&D. Also, if timing detectors based on other principles, e.g. solid state detectors, demonstrate
good performance and acceptable properties (e.g. radiation hardness) they can supplement, or possibly 
replace, the Quartic detectors.



%\subsubsection{Summary of Quartic Detectors}

%The L-bar Quartic design satisfies the requirements of edgelessness (within about 100\,$\mu$m), 
%sufficient radiation hardness, ability to measure
%several protons within a bunch crossing (time spread $\sigma = 150$\,ps) if in separate bars, and to be 
%active every 25\,ns (the bunch separation). 
%We plan to construct and install a pair of L-bar Quartic modules, with SiPM photodetectors, in a 
%RP on each arm, and use them in 2015
%to assess their performance in realistic conditions, as well as for physics in the low pileup runs. 
%The modules will be constructed at Fermilab 
%and the signals from the
%SiPM board sent to a local DAQ.% (which will be the responsibity of the Lisbon Group).

%Further development will continue to improve their time resolution and possibly the spatial segmentation. 
%Therefore R\&D will continue, and improved versions could be ready for installation at the end of 2015.  


\subsubsection*{Readout System of the Cherenkov Detectors}
\label{sec:timing_electronics}

The task of the readout system is to provide time and amplitude measurements of
the pulses generated by the photosensors associated to the Cherenkov detectors, and to transmit the digitized data to 
the data acquisition system. 
%Given the similar characteristics of the Quartic
%and Gastof detectors, the readout system is expected to be suitable for both
%detectors.

The Cherenkov timing detectors are composed of a number of modules installed in
one or more RP. The readout system follows the same
modularity, and is composed of independent units (readout module) interfacing to the CT-PPS
DAQ/Trigger system. Each readout module has $64$ channels suitable for use with
the baseline Quartic module ($20$ channels), but also with possible Quartic modules with finer granularity.
% and with the Gastof $8\times8$ anode MCP-PMT.

%Each electronic channel must be able to handle very fast pulses (rise time $\sim 1$ ns) from
%silicon photomultipliers or micro-channel plates. The photon yield of the
%Cherenkov signals per channel is %range from $1$ photon in the case of Gastof MCP to
%about $100$ photons in the case of Quartic.
%The SiPM gain is of the order of $10^{6}$ while the MCP-PMT will be operated at
%about 10 times lower gain to limit the total charge collected (see~\cite{ctpps-tdr}, Section~5.3).
%Therefore the dynamic range of the input signals is in the range of 20\,fC to 20\,pC.

%The timing precision of the readout system is required to be 20\,ps, which,
%combined with a similar precision of the Quartic detector, would yield 30\,ps
%precision per module, and global precision (two modules) of about 20\,ps. When
%associated to one Gastof detector, assuming 7 photoelectrons per proton and a
%precision of 30\,ps per MCP-PMT channel, we may estimate that the readout system would
%provide a measurement with 15\,ps precision.
 
The readout system is also required to provide the measurement of the input pulse amplitude. 
While this measurement is not directly used in the reconstruction of
the collision vertex, the knowledge of the amplitude is mandatory for detector
calibration, time corrections (e.g. ``time-walk'') and pulse pile-up rejection.

The readout system is required to have double hit resolution better than 25\,ns, suitable for operation with 25\,ns bunch separation without loss of
efficiency, and to sustain a maximum rate of 6\,MHz
per channel, corresponding to a maximum channel occupancy of 20\% at 25\,ns
LHC beam operation, averaged over all channels. While the average occupancy of the Quartic channels ($3\times3\rm\,mm^{2}$ quartz bars) is 20\% for average pile-up of
50 events, the highly non-uniform occupancy of the detector (the
occupancy of the innermost channels reach 70\%) induces a
significant readout inefficiency for a number of pile-up events larger than 25.
%To sustain twice this value, as foreseen in Run 2, a fine-granularity Quartic
%version will be required. In the case of the Gastof detector, a channel occupancy 
%smaller than 20\% is expected.

The readout system is required to provide on-detector L1 trigger matching, allowing extraction 
of the detector data in a time window around the L1 time, local event building
and data transmission to the DAQ system. 
The data rate of a readout module, assuming readout 
of 10 channels after zero suppression, 3 bunch crossings time window, 32 bit
event data per channel, and 100\,kHz L1 rate, is estimated to be 100\,Mb/s.

The timing detector readout system is expected to provide hit information and
time measurement at the bunch crossing rate to be used by the trigger system. By
combining the information from the two PPS arms, the L1 can estimate the
z-vertex coordinate, allowing to select events in the tails of the z-vertex
distribution where the pileup density is smaller. This capability would provide
a reduction of the L1 rate of high cross-section processes so that it fits
within the L1 rate constraints, selecting at the same time the events less affected by pileup. 
The trigger requirement implies the use of a low latency TDC delivering
conversion data at the bunch crossing rate.

In order to achieve the desired time resolution, the front-end timing
electronics must be located in the RPs or a nearby region (1-2\,m
distance). This raises issues of radiation tolerance since the
radiation levels in the RPs, in the region 200\,m from IP, are expected to be 100\,Gy and $10^{12}$ neq/cm$^2$ for 100\,fb$^{-1}$ of integrated luminosity.
%Together with machine
%experts, we have explored the feasibility of digging a hole in the
%tunnel floor concrete below the timing RPs, which would provide a substantial
%reduction of the radiation exposure. While this possibility is technically feasible, the
%proposal could not be accommodated in the present LHC LS1 schedule but would be
%possible if necessary in the winter technical stop 2015-16.

\paragraph*{System Design}

The main guideline in the design of the timing detector readout system was to
reuse well known components with adequate performance, allowing to streamline the design and implementation of the system 
so that it may be possible to evaluate the timing detectors in the LHC beam in 2015.

We have therefore decided to base our system on the amplifier-discriminator
NINO and the time-to-digital converter HPTDC. Both chips have been developed by
CERN's microelectronics group for the LHC experiments. The HPTDC chip is used in the CMS muon system, while the NINO 
and HPTDC chips are associated in the time-of-flight detector of the ALICE experiment. 
These chips are now widely used in many applications, including PET Time-of-Flight. 

The EndoTOFPET-US collaboration\footnote{This 
project  have  been  funded  by  the  European  Union  7th  Framework  Program  (FP7 / 2007-2013) under Grant Agreement No. 256984 (EndoTOFPET-US)} has studied the
time resolution of the NINO-HPTDC readout chain, using laser pulses detected by $3\times3$\,mm$^{2}$ SiPMs (Hamamatsu MPPC) with
SPAD size of $50\,\mu$m~\cite{Gundacker}.
The measured time resolution as a function of the number of photo-electrons is
shown in Figure~\ref{fig:nino_hptdc_resolution}.
For 100 photoelectrons a resolution better than 20\,ps is achieved.

\begin{figure}
\centering
\includegraphics[width=100mm]{figs/detector/nino_hptdc_resolution.pdf}
%\vspace*{5cm}
\caption{Time resolution of laser pulses as a function of the number of
photo-electrons measured with MPPC and the NINO-HPTDC electronics chain.}
\label{fig:nino_hptdc_resolution}
\end{figure}

The NINO amplifier-discriminator is implemented in a 8 channel ASIC. 
%A newer version with 32 channels developed by an external group is also suitable.
The time binning and number of channels of the HPTDC ASIC is configurable. In our case we use 
the HPTDC high-resolution mode, which provides 8 channels with 25\,ps time
binning.
The timing readout system is designed to be integrated in the common CT-PPS DAQ and Control 
system, based on the CMS Pixel FED and FEC boards. The FED board provides input
to 400\,Mb/s optical links transmitting detector data, builds event packages and
transmits them to the central DAQ.
The FEC board transmits fast controls (LHC clock, L1 and fast signals) to the detector, as 
well as front-end configuration data. We plan to use the same components used in the Pixel 
detector to implement the on-detector interface to the FED and FEC board, namely the  
transmission and reception optical hybrids and the CCU control chips.

Physically, the timing readout system is implemented in two electronics boards:
%(see Figure~\ref{fig:readoutsystemdiagram}):
1) the frontend board, housing 8 NINO chips and installed in the RP, 
which receives the SiPM signals transmits the LVDS output on the feed-through
connector; 2) the digital board, which receives the LVDS output of the discriminators and
houses 8 HPTDC chips. The digital board integrates a radiation resistant FPGA to
serve as readout controller of the HPTDC chips, and provides on-board connectors to the opto-hybrid mezzanines (PoH and DoH). 
If required, the 
digital board could be installed a few meters away of the RPs in a radiation protected place.

%\begin{figure}
%\centering
%\includegraphics[width=150mm]{figs/detector/readoutsystemdiagram.pdf}
%%\vspace*{5cm}
%\caption{Diagram of the timing readout system.}
%\label{fig:readoutsystemdiagram}
%\end{figure}

%--------------------------
%\input{ctpps_el.tex}     
%-------------------------- 

\subsection{Pixel Tracking System}
\label{sec:silicon}
%
The key requirements for the CT-PPS tracking system are:
\vspace{-0.5\baselineskip}
\begin{itemize}
\item Efficient pixel based tracking as close as possible 
to the sensors physical edge, providing hit resolution better than 
30~$\mu$m.
\item Radiation hardness: 
a design figure of $5\cdot 10^{15}$~protons/cm$^2$ for 100~fb$^{-1}$ of
integrated luminosity is required (Figure \ref{fig:ProtonFluence}).
\item Reliable operation at the highest LHC luminosity.
\end{itemize}
\vspace{-0.5\baselineskip}

\begin{figure}[h!]
\begin{center}
\includegraphics[width=0.6\linewidth]{figs/detector/ProtonFluence_Pythia6_s-1622.pdf}
%\vspace*{5cm}
\caption{Simulated proton fluence in the tracking station at 204~m from 
the IP for the integrated luminosity of 100\,fb$^{-1}$. The rectangle 
indicates the detector surface transverse to the beam assuming a detector 
tilt angle of 20$^{\circ}$. The ellipse shows the 15 sigma beam contour.
In the detector edge a value of the order of $5\times 10^{15}$\,p/cm$^2$ 
is obtained. This value is compatible with the extrapolation from TOTEM data.}
\label{fig:ProtonFluence}
\end{center}
\end{figure}

{\bf to be rephrased}
Since the construction of the original pixel tracking systems for 
the LHC experiments, there has been considerable progress in 
silicon sensor technology. Both CMS and ATLAS have pursued improved 
pixel designs for the high-luminosity upgrades of the LHC. 
These ongoing R\&D efforts have already achieved two proven sensor 
designs that meet the needs 
of CT-PPS and can be produced by industry: 3D and planar slim-edge 
silicon pixel sensors. Both types of sensors are being installed in 
the new Insertable Barrel Layer (IBL) of the ATLAS vertex 
detector~\cite{ATLAS_IBL}.

3D sensors~\cite{parker-3d} consist of an array of columnar electrodes (radius 
$\sim$5\,$\mu$m) of both doping types that penetrate through the 
silicon bulk perpendicularly to the surface, as shown in 
Figure~\ref{fig:silicon-3D}. The bulk is usually 
of type p. Junction n-type electrodes are read out on the 
front side of the sensor while ohmic p-type electrodes are 
connected on the back side for applying the bias voltage. 
This structure decouples the inter-electrode distance from the 
sensor substrate thickness, allowing to reduce the drift path 
of the charge carriers without decreasing the total generated charge. \\
The close electrode spacing provides several advantages compared to 
the planar sensor design:
%\vspace{-0.5\baselineskip}
\begin{itemize}
\item low full depletion voltage ($\sim$10\,V),
\item fast charge collection time, 
\item reduced charge-trapping probability and therefore high radiation hardness. 
\end{itemize}
%\vspace{-0.5\baselineskip}

%As a result, 3D detectors are emerging as one of the most 
%promising technologies for the innermost layers of tracking devices for 
%the foreseen upgrades of the LHC.
%A very interesting feature of 3D technology is the possibility of 
%realizing the so-called ``active edge''~\cite{active-edge}, 
%i.e. a deep trench all around 
%the sensor that reduces the dead region to a few microns from the 
%physical edge of the device, compared to the hundreds of $\mu$m for 
%standard planar detectors.

\begin{figure}
\centering
\begin{center}
\includegraphics[height=1.5in]{figs/detector/3D_Structure.png}
%\vspace*{5cm}
\end{center}
\caption{Sketch of a 3D sensor.}
\label{fig:silicon-3D}
\end{figure}

{\bf to be rephrased}
The baseline CT-PPS tracking system is based on  
3D pixel sensors, produced either by FBK (Trento, Italy)~\cite{FBK} or CNM (Barcelona, 
Spain)~\cite{CNM}, which we think provide the best performance in terms 
of active region and radiation hardness. 
These companies have already produced 200~$\mu$m slim-edge 
3D sensors for the IBL project with satisfactory yield. 
However, for CT-PPS we would like to pursue the option with 
a 100~$\mu$m, or better, slim-edge design, where the active region 
of the sensor is as close as 100~$\mu$m to the edge. 
Since such slim edges have not yet been produced, we mitigated 
our schedule risk by designing the CT-PPS tracking system 
to allow rapid installation, or replacement, 
of the unit during a LHC technical stop. 


As a backup solution, we have identified a second sensor concept, 
a slim-edge planar design 
produced by CIS (tested by ATLAS) and SINTEF(tested by CMS), based 
on a more mature fabrication process. We have designed 
the CT-PPS sensor readout and packaging to accept either sensors 
as a drop-in replacement. 

The chosen configuration for the tracking system consists of two 
detector units in each arm, for a total of four detector units. 
These are the horizontal RPs located at $\sim$210\,m.
Each station will contain one stack of silicon tracking detectors. 
Each stack will consist of six planes, where each plane contains 
a 1.6$\times$2.4\,cm$^2$ pixel sensor read out by six PSI46dig readout chips
ROCs~\cite{CMS_digROC}. Each ROC reads 52$\times$80 pixels with 
dimensions 150$\times$100\,$\mu$m$^2$. Given the small area of the detector,
covered by a small number of individual sensors, we have chosen a number of
planes that provide confortable redundancy making the system resilient
to possible failures.  The design of 
the front-end electronics and of the DAQ is based on that developed for the 
Phase 1 upgrade of the CMS silicon pixel 
detectors~\cite{Ph1-TDR}.

The resolution of the x-coordinate is determined by the sharing of charge in
the pixel clusters, which depends on the detector tilt angle in the x-z plane.  
While this parameter is not yet defined, test beam results with similar sensors 
indicate that for an angle of $<$20 degrees the two-pixel clusters have resolution
of the order of 10\,$\mu$m.  Since there is no tilt in the y-z plane, the
resolution of the y-coordinate is of the order of 30\,$\mu$m.

Recently (May 2014), in a test beam at Fermilab, seven un-irradiated 
({\bf define FBK,1E})
FBK 1E 3D sensors, processed in the framework of the ATLAS IBL 
production~\cite{3DATLAS-production}, with 200~$\mu$m slim 
edges~\cite{slim-edge}, have been tested coupled to the new PSI46dig ROC,  
developed for the Phase 1 upgrade of the CMS pixel tracking 
detectors. 
%Data analysis is still ongoing but preliminary
%results are very promising. The possibility to lower the 
%channel thresholds down to $\sim$2500~e$^-$ and to trim their values 
%more accurately made it feasible to obtain efficiencies above 99.5\%, 
%with full charge collection at bias voltages above $\sim$15~V. 
Figure~\ref{silicon3DEffCell} shows the two-dimensional map of the 
cell efficiency for one of these sensors at normal beam incidence (left panel) 
and with the detector tilted by 5 degrees with respect to 
the beam axis (right panel). 
%To increase the statistics, all cells have been added together, assuming they have a similar behaviour.    
Low efficiency structures, corresponding to the position of the electrodes, 
are clearly visible in the left plot. These structures, due to the fact that 
in FBK sensors the electrodes are empty and do not produce charge, 
disappear in the right plot, proving that a tilt of 5 degrees is 
sufficient to fully restore sensor efficiency. 
   
\begin{figure}
\centering
\begin{center}
\includegraphics[height=1.6in]{figs/detector/CellEff_3D_0deg_5deg.png}
%\vspace*{5cm}
\end{center}
\caption{Cell efficiency map for the sensor FBK 11-37-02 obtained using 
normal incident tracks (left panel) and 5$^{\circ}$ inclined tracks (right panel). 
These measurements were performed at room temperature and with a 
bias voltage of $|V_{bias}|$~=~30~V.}
\label{silicon3DEffCell}
\end{figure}


%\input{ctpps_pixel.tex}


\subsubsection*{The Readout System}

The readout of the pixel detector is largely based on components developed in the framework of the CMS Pixel 
Upgrade Phase 1 readout project. 
%This readout chain has been proven to work efficiently. 
Most components
are currently at an advanced test stage and/or in final production. 

%In this section, an overview of the readout system of the pixel detector is given shortly with special 
%emphasis on CT-PPS specific points. 
Extensive documentation of each component can be obtained elsewhere~\cite{Ph1-TDR}.

%The complete readout chain of one detector package is shown in Figure~\ref{silicon:readout}. 
By convention a detector package is a set of six modules, one for each sensor present in 
a RP. There are in total four detector packages.
The specific CT-PPS elements in the readout system are the six RPix Modules (Roman Pot PIXel Modules) 
and the RPix Portcard. 
The low voltage system and high voltage system are part of the low voltage and high
voltage system of TOTEM, already in place.
The backend DAQ electronics, to be installed in the service cavern, is being actively developed  
by CMS as part of the Pixel Upgrade Phase 1 project.

%\begin{figure}[htb!]
%\centering
%\includegraphics[height=4.2in]{figs/detector/readout.pdf}
%%\vspace*{5cm}
%\caption{Detector readout and control strings. All components up to PP1 are in the LHC tunnel, while
%         FEDs and FECs are in the service cavern.}
%\label{silicon:readout}
%\end{figure}

Each RPix Module consists of a flexible hybrid circuit hosting: a silicon sensor, six ROCs ``bump-bonded'' to the silicon sensor, and one Token Bit Manager  (TBM) chip. 
The ROC is responsible for charge collection, charge discrimination and data sparsification. 
%Two slightly different versions of the chip, named V2.1 and V2.1b, are suitable: 
%which version to use is currently under evaluation.

The TBM is responsible for reading out the six ROCs in the module (it can manage up to 16) using a token ring protocol
and serialising the data over a single output line.
The TBM %versions suitable for this application, named TBM08a and TBM08b, 
manages two token bit ring protocols 
at the same time, multiplexing the two data streams on the same output line before encoding the data stream.
% using a 4B/5B NRZI schema.
The net result is an uplink data stream running at 400 Mb/s. 
Dispatching these high speed signals on the flexible hybrid without degrading them
is one of the major design requirements of the RPix Module, together with the need to
deliver the high voltage to the sensor safely. 

The RPix Portcard accomplishes a variety of tasks. The board receives the output data from six RPix
modules  and retransmits them on six optical fibres towards DAQ modules, using a POH7 opto-electrical 
converter mezzanine card~\cite{POH}.
This board also receives fast configuration commands from the Pixel FEC via optical fibres, translates these 
signals using detector optical receivers (DOH) and dispatches them to the modules. 
These functionality are similar to those of the Forward Pixel project portcard developed by Fermilab.
Moreover the RPix Portcard integrates other components such as the radiation sensors, part of the TOTEM DCS 
radiation monitoring system, and the CMS Tracker Optical Control Link components which are
capable of receiving and decoding the commands sent from the Tracker FEC. 
Finally, the newly developed DC/DC converters~\cite{DCDC1}, developed by CMS, are installed on the board, 
in order to generate the different voltages needed by the portcard itself and by the attached modules.

For the backend DAQ system, the plan is to use the new uTCA crates and boards developed for the Pixel Upgrade 
Phase 1 project. A fallback solution, using VME electronics, is available in case the baseline solution could suffer 
long delays.

It should be noted that the tracking front-end based on the
CMS pixel readout chip PSI46dig chip does not have trigger outputs and
therefore can not be integrated in the L1 Trigger.
%\input{ctpps_pixel.tex}

\input{detectors/afp_yr.tex}
 
\input{detectors/yellow_lhcb.tex}



 


==> detectors/table_forw.tex <==
  \section{Forward detector coverage for LHC Experiments}
  
  The following table provides information on the coverage of LHC detectors with $|\eta| >$ 5.
   
\begin{table}[ht]
\begin{center}
\begin{tabular}{|c|c|c|c|c|}
\hline
\hline
Experiment  & Detector & Hardware  &  Acceptance    &  Comment\\
            &          & Tecnology &           &    \\
\hline
ATLAS & LUCID  &  Gas Cherenkov tubes  & 5.9 $<|\eta|<$ 6.0   & \\
  & ALFA   & Scintillating fibres  &    & Forward proton tracking   \\
  &     &    &    & $0<\xi<0.2$ high-$\beta^*$   \\
  & ZDC    & Quartz rods, tungsten    &$|\eta|>$ 8.3  &   Neutrals only\\
  & AFP    &  Tracking: Silicon  &  &   Forward proton tracking \\
  &   &      Timing:Quartz Cherenkov  &   & $\approx 0.03<\xi<0.2$  low-$\beta^*$\\
\hline
 ALICE & ADA    & Scintillator   &-7.0 $<\eta<$ -4.8     &  \\
  & ADC    & Scintillator   &4.7 $<\eta<$ 6.3    &  \\
\hline
 CMS   & CASTOR & Quartz plates, tungsten & -6.8 <\eta< -5.2    &  \\
   &  FSC   & Scintillator   &6 $<|\eta|<$ 8  &    \\
    & ZDC    &  Quartz fibres, tungsten  & $|\eta|>$ 8  & Neutrals only\\
 TOTEM & T1     & Cathode Strip Chambers   &3.1 $<|\eta|<$ 4.7    & \\
  & T2     & GEM Chambers  & 5.3 $<|\eta|<$ 6.5    & \\
  & RP &  Silicon  &  &    Forward proton tracking   \\
  &  &    &    & $0<\xi<0.2$ high-$\beta^*$   \\
 CMS+TOTEM & CT-PPS  & Tracking: Silicon  &    & Forward proton tracking \\
           &           &Timing: Quartz Cherenkov     &    &  $\approx 0.03<\xi<0.2$  low-$\beta^*$\\
\hline
 LHCb & HERSCHEL & Scintillator  &  5 $<|\eta|<$ 8   & \\
 
   \hline
 \end{tabular}
 \\[4.0mm]
 Table 1 : Summary of very forward detector coverage of LHC experiments \\
  in Run II. Several numbers are approximate. \\ 
 \end{center}
  \label{sigmas}
\end{table}


==> introduction/conclusion.tex <==

\section{Conclusion}
\label{sec:forwardacceptanceconclusion}

The geometric acceptance for vertical (ALFA, at 237--245 m) and horizontal (AFP, at 204--212 m) Roman pot detectors is parametrised as a function of the fractional momentum loss ($\xi$) and \pt\ of the scattered proton at $\sqrt{s} = 14 \TeV$. Proton transport is performed with the \textsc{MAD-X} application using relevant LHC optics files for collision ($\beta^* = 0.55$ m) and high-$\beta^*$ ($\beta^* = 90, 1000$ m).

A data driven estimation of beam induced backgrounds in TOTEM is presented to quantify the probability of forward proton tags from beam halo or collision debris. A zero bias data sample is corrected to remove hits due to physics using data from the TOTEM T2 telescope and Monte Carlo simulation. The remaining background is scaled to different running scenarios.

==> introduction/runcond_tab.tex <==
\begin{table}[ht]
\begin{center}
\begin{tabular}{|c|c|c|c|c|c|c|p{4cm}|}
\hline
\hline
Conditions & $\beta^*$  &  N  & N$_b$ & $\mu$  & L & L$_{int}$ &  Physics \\
 & [m] &  [10$^{11}$ p/b] & &  (pileup) &[cm$^{-2}$s$^{-1}$] &  [24h] &   \\
\hline
\multirow{2}{*}{LOW}    & $\geq$ 1000 & 0.7 & 2        & 0.004 & 10$^{27}$          & 0.1/nb    &  $\sigma_{tot}$; Coulumb region \\
                        & 19          & 0.1 & 40       & 0.01  &  5$\cdot$10$^{28}$ & 4.8/nb    & Lhcf Run; Multiplicity; energy flow; Inelastic cross section \\
\hline\multirow{3}{*}{MEDIUM} & 19          & 0.7 & 40       & 0.4   &  2$\cdot$10$^{30}$ & 0.17/pb      & High cross section diffraction \\
                        & 90          & 0.7 & 156--700 & 0.1   &10$^{30}$--10$^{31}$& 0.2--1/pb & $\sigma_{tot}$; low mass diffraction; Hard diffraction\\
                        & 90          & 1.5 &      700 & 0.6   &5$\cdot$10$^{31}$   & 4.4/pb    & Glueball searches; CEP \\                        
\hline\multirow{2}{*}{HIGH}   & 0.5         & 1.15& 2800     &       &                    &           &    LHCb programme   \\
                        & 0.5         & 1.15& 2800     & 30    &         10$^{34}$  & 1/fb      &  Exclusive dijets, anomalous coupling      \\
 \hline
 \end{tabular}   
 \end{center}
 \caption{Summary of the machine parameters for the different running conditions. } 
  \label{runcond}
\end{table}


==> introduction/tot-acc.tex <==
 \begin{figure}[htb]
\centering
\includegraphics[height=2.7in, width=0.49\linewidth]{figs/introduction/acceptance_90.pdf}
\includegraphics[height=2.7in, width=0.49\linewidth]{figs/introduction/acceptance_2.pdf}
\caption{Geometric acceptance of the TOTEM-RP detectors (vertical and horizontal) as a function of the proton relative energy loss ($\xi$) and its squared four-momentum transfer ($t$) 
for different LHC optics settings (left, $\beta^*$=90\,m; right, low-$\beta^*$),
at the beam energy of 7 TeV and at detector distance from the beam corresponding to 10$\sigma$+0.5\,mm.}
\label{fig:totemacc}
\end{figure}

Similar considerations can be done for the acceptance in the leading proton detectors in IP5.
The detailed acceptance studies of the TOTEM and CT-PPS detectors have been published already elesewhere (\cite{totem-upgrade-tdr,ctpps-tdr}).
As example in Fig.~\ref{fig:totemacc} is shown the acceptance for high (90\,m) and low beta optics, for both vertical and horizontal detectors.
 




